Learning to Rectify for Robust Learning with Noisy Labels

Label noise significantly degrades the generalization ability of deep models in applications. Effective strategies and approaches, \textit{e.g.} re-weighting, or loss correction, are designed to alleviate the negative impact of label noise when training a neural network. Those existing works usually rely on the pre-specified architecture and manually tuning the additional hyper-parameters. In this paper, we propose warped probabilistic inference (WarPI) to achieve adaptively rectifying the training procedure for the classification network within the meta-learning scenario. In contrast to the deterministic models, WarPI is formulated as a hierarchical probabilistic model by learning an amortization meta-network, which can resolve sample ambiguity and be therefore more robust to serious label noise. Unlike the existing approximated weighting function of directly generating weight values from losses, our meta-network is learned to estimate a rectifying vector from the input of the logits and labels, which has the capability of leveraging sufficient information lying in them. This provides an effective way to rectify the learning procedure for the classification network, demonstrating a significant improvement of the generalization ability. Besides, modeling the rectifying vector as a latent variable and learning the meta-network can be seamlessly integrated into the SGD optimization of the classification network. We evaluate WarPI on four benchmarks of robust learning with noisy labels and achieve the new state-of-the-art under variant noise types. Extensive study and analysis also demonstrate the effectiveness of our model.

==> 1-abstract.tex <==
%Meta-learning provides an effective learning paradigm to leverage prior knowledge from experienced tasks that enables fast adaption to new tasks with improved performance. 
%The crux of meta-learning for few-shot learning is to design a meta-learner that effectively accrues knowledge during the learning process to improve the performance of a base-learner on new tasks with limited data. 

%Deep learning relies on large amounts of trusted data, but the noise prevails in real situations can be detrimental to the performance of the algorithm. Assigning weights or other adaptation methods on training data with noise is a common approach to this problem. In this paper we propose a probabilistic adaptation method based on meta-learning to reduce the negative impact of incorrect labels. Our experiment results show that our method is effective even with a fairly high noise rate, and it has achieved results that outperform the state-of-art method.


Label noise significantly degrades the generalization ability of deep models in applications. Effective strategies and approaches, \textit{e.g.} re-weighting, or loss correction, are designed to alleviate the negative impact of label noise when training a neural network. Those existing works usually rely on the pre-specified architecture and manually tuning the additional hyper-parameters. In this paper, we propose warped probabilistic inference (WarPI) to achieve adaptively rectifying the training procedure 
for the classification network within the meta-learning scenario. In contrast to the deterministic models, WarPI is formulated as a hierarchical probabilistic model by learning an amortization meta-network, which can resolve sample ambiguity and be therefore more robust to serious label noise. 
Unlike the existing approximated weighting function of directly generating weight values from losses, our meta-network is learned to estimate a rectifying vector from the input of the logits and labels, which has the capability of leveraging sufficient information lying in them. This provides an effective way to rectify the learning procedure for the classification network, demonstrating a significant improvement of the generalization ability. Besides, modeling the rectifying vector as a latent variable and learning the meta-network can be seamlessly integrated into the SGD optimization of the classification network. We evaluate WarPI on four benchmarks of robust learning with noisy labels and achieve the new state-of-the-art under variant noise types. Extensive study and analysis also demonstrate the effectiveness of our model.     

==> 2-introduction.tex <==
% Recent years, deep learning has achieved amazing results in image classification, semantic segmentation and many other domains, while most algorithms theoretically require a large amount of trusted training data to ensure the output is reliable. But sometimes it is hard to obtain such a lot high-quality data that meet the training requirement. One way to reduce cost is to crawl data from web pages or label data via automated system. Obviously these approach will produce noise. And for some domains, the label itself has ambiguities, such as complex semantic segmentation problems and questions defined by subjective consciousness. Although the deep network has the characteristics of resisting noise to a certain extent, it still tend to overfit to those noisy data, especially these complex and powerful model, which will be quilt harmful. Based on the above reasons, learning from noisy data has been a hot research topic for a long time .
% % \begin{figure*}[t]
% % 	\centering
% % 	\includegraphics[width=.95\linewidth]{./figs/fig1.pdf}
% % \label{fig:frame}
% % 	\vspace{-2mm}
% % 	\caption{The learning framework of our meta variational random features.}
% % 	\vspace{-4mm}
% % \end{figure*}

% In many cases, there exist data with corrupted labels that we do not know in the training data. To reduce the negative impact of noise factors on the performance of the model, an intuitive approach is to use some determinate clean data to guide the performance of noisy data. Although finding and fixing all the corrupted data in the training set is almost impossible, it is feasible to construct a completely clean meta-data set which is much smaller than the training data set. In the meta-data set, each class may only have a few dozen or hundred of samples. 

% In order to achieve this correction process, we do not directly use the original prediction vector (output of the classification network), but introduce a fully connected network as the meta-learner to obtain a correction vector to act on the original prediction vector, and then use the corrected prediction vector for training. From the meta-model, the original prediction vector and its corresponding label is mapped to the correction vector. It is worth noting that we chose to generate the distribution of the correction vector instead of a specific vector，which can increase the generalization ability of the model.    

% To reduce the impact of corrupted samples on algorithm performance, most existing works utilize the loss between the output of the classifier and the corresponding label to obtain the sample’s weight. The weight act on the parameters’ update process, and in most cases, it decreases as the loss increases to reduce the impact of noise. This rule is established not only on the manually set mapping function like AdaBoost and focal loss, but also on the automatically generated mapping model, for example, Meta-Weight-net. Although using the loss to generate the weight corresponding to the sample has achieved great efficiency, there still exists some deficiencies. (1) Only use loss as the variable for generating weights, ignoring some valuable structural information of the sample. Meanwhile, the distribution of the original label and the confused label are not completely independent, similar classes are usually more likely to be mislabeled. (2) Experience has shown that corrupted samples have a certain value at the early training, and giving smaller weights to these data the entire training process cannot make full use of these corrupted samples. (3) The deterministic function unable to model the uncertainty of the problem, which could cause bias especially in few shot cases.

% We make three contributions in this paper as follows. (1) We propose a classification correction probabilistic framework based on meta-learning. We propose a classification correction probabilistic framework based on meta-learning. We introduce a correction vector, which works on the original prediction vector. We spliced the original prediction vector with the one-hot  label vector to generate the correction vector. This helps us to use the structural information of the data, while considering the category information. (2) We utilize the Bayesian probability model to generate the distribution of correction vector, viewing each item of the correction vector as a latent variable of the credibility of the pretend probability of each class obtained by classification network. The Bayesian probability model can model the uncertainty of the prediction process, especially the ambiguity of the data for the few shot learning. In this function we use a small amount of meta-data to guide the update of meta-learner, therefore our method would be more robust by introducing the probabilistic model. (3) Using the correction vector to correct the original prediction vector can make better use of the corrupted data and improve efficiency, compared to sample weighting methods.

% To evaluate the effect of our method, we conduct experiments on the CIFAR10, CIFAR100 and Clothing1m data sets. The experimental results shows that our method exceed the state of art method in many indicators.

Learning from noisy labels for deep models is a challenging problem in practice~\citep{angluin1988learning,frenay2013classification}. Since data noise is ubiquitous in the real world, collecting training data with clean labels would be resource-intensive, especially for some domains with ambiguous labels, such as semantic segmentation. As noisy labels are corrupted from ground-truth labels, the robustness of  
learned deep models would be degraded under the circumstance of high noise ratios, due to its high capability of fitting noisy labels~\citep{zhang2017understanding}. %This situation would be severe Modern deep models with sophisticated structures tend to overfit to training data~\citep{zhang2017understanding} demonstrating irritating vulnerability to label noise. 
%especially these complex and powerful model~\citep{zhang2017understanding} vulnerable  heavily rely on the large-scale training set The performance of modern deep models heavily rely on the large-scale training set. since training data collected in reality is often difficult to guarantee to be completely clean. Although the deep network has the characteristics of resisting noise to a certain extent, it still tend to overfit to noisy data, especially these complex and powerful model~\citep{zhang2017understanding}, which will be quilt harmful. Ensuring the used data is all trusted would be resource-intensive and for some domains, the label itself has ambiguities, such as complex semantic segmentation problems and questions defined by subjective consciousness. Thus, learning from noisy data remains quite challenging. 

To reduce the impact of corrupted labels in supervised learning tasks, two effective strategies of sample re-weighting and loss correction are introduced in previous methods. The key idea of the former is to down-weight training samples that are likely to have incorrect labels by a weighting function. Existing weighting functions~\citep{kumar2010self} commonly leverage the empirical loss of a sample as the input to estimate the corresponding weight value and monotonically decrease the weight as the loss increases. Those functions can be pre-designed using certain prior knowledge~\citep{zadrozny2004learning} or dynamically optimized in each iteration of the training process~\citep{khan2017cost,jiang2018Mentornet}. 
%Using training loss to generate weights for the corresponding samples is a common strategy, some of them tend to make the algorithm not fit samples with large loss, as they are more likely to be outliers. Such as curriculum learning methods  Mentornet~\citep{jiang2018Mentornet}, it learns another neural network (MentorNet) as curriculum to supervise the base network (StudentNet) and provides a sample weighting scheme. 
The strategy of loss correction focuses on changing the form of the loss function. 
%Pioneer works~\citep{sukhbaatar2015training} attach a noise layer to the classification model introduce a confusion matrix calculated by. The confusion matrix characterises the transform probability between true and corrupted labels in the training data. Thus, the predicted label are corrected by the confusion matrix to be closer to the noise label, thus reducing the overfitting of the model to the biased samples. 
The straightforward method is to correct corrupted labels via a confusion matrix~\citep{ryutaro2019learning}. This matrix characterises the transform probability between true and corrupted labels in the training data, where the annotations can be corrected accordingly and the model would be trained on a cleaner dataset. 
Although these strategies can eliminate the impact of noisy labels to some extent, there still exist two limitations in practice. Firstly, the form of the weighting or correction functions need to be specified manually under certain assumptions on data, which is infeasible in the real world. Secondly, hyper-parameters in these functions are usually tuned by cross-validation, impairing stability of performance of trained models.


Methods based on meta-learning for noisy labels have emerged recently~\citep{ren2018learning,chen2015webly,hendrycks2018using}. These methods essentially formulate the task as a meta-learning problem. By constructing a small completely clean data set called meta-data set, an adaptive weighting or correction meta-function is learned from the meta-data set, which can avoid manually tuning of hyperparameters~\citep{ren2018learning} and omit the assumption of the function form~\citep{shu2019meta}. %~\citep{ren2018learning} proposed a meta-learning based approach through an iterative training process, and Meta-Weight-Net~\citep{shu2019meta} utilize a multi-layer perceptron(MLP) as the loss-to-weight mapping function, updated through meta data. Due to the powerful fitting ability of MLP, it can be very close to the complex mapping function of the real situation, so as to adapt to different type of noise data. For loss function correction methods, ~\citep{chen2015webly,hendrycks2018using} show that the use of meta data encourages algorithm convergence to the real confusion matrix. Another strategy is to correct the wrong label to soft label, \citep{yichen2020softlabel} implements this mapping process under the guidance of meta data. 
Although existing meta-learning-based approaches have achieved great efficiency and significantly improved robustness of prediction models, there still exist two deficiencies. 
(1) Those methods built with the deterministic model usually neglect sample ambiguity~\citep{finn2018probabilistic}, even with the effective prior, there might not be enough information in the sample to estimate the weight or rectify the loss with high certainty. It would be desirable for the meta-function to propose multiple potential solutions to the ambiguous weighting or rectifying task. (2) The meta-function, such as the meta weighting function, utilizes the training loss as the input to estimate the corresponding weights, which is deficient in exploiting structure information in the prediction.
%    ignore the distribution relationship of classes. As for loss correction methods,  as the classes of training data increasing, the confusion matrix becomes too large to calculate. 
%, Data re-weighting methods
%In this paper, we propose a meta-learning based warp method under a probabilistic model that can correct the prediction vector of the classifier to be close to the potentially corrupted labels. Our method consist of two models: base-model as classifier to calculate the logits, and meta-learner to compute the rectifying vector. We utilize the logits and the corresponding label as input to the meta-learner to compute the rectifying vector. It helps us to use the structural information of the data itself, while considering the category information as well. It is worth noting that we chose to generate the distribution of the rectifying vector instead of a determined value, which can increase the generalization ability of the model. The probability model can model the uncertainty of the prediction process, especially the ambiguity of the data for the few shot learning, therefore our method would be more robust by introducing the probabilistic model.

In this paper, we build a hierarchical probabilistic model, warped probabilistic inference (WarPI), to achieve adaptively learning from the meta-data set for noisy labels in the meta-learning scenario. In contrast to the deterministic models, we treat the rectifying vector as the latent variable. The training process for classification networks can be rectified effectively by learning an amortization meta-network. The meta-network estimates the distribution of the rectifying vector, which can deal with sample ambiguity by modeling its uncertainty and be more robust to serious label noise. Unlike existing meta-functions to leverage the training loss as input, we design a more powerful meta-network that generates the distribution from the input of the logits and labels, which demonstrates a significant improvement of the generalization ability in our experiments. Our WarPI can be seamlessly integrated into the SGD optimization of the classification network and show favorable properties to alleviate the impact of noisy labels. 


Contributions can be summarized in three aspects. \textbf{(1) Our WarPI is the first probabilistic model to resolve label noise within the meta-learning scenario. (2) We design a powerful amortized meta-network to estimate the distribution of the rectifying vector from the input of labels and predicted vector. (3) WarPI can be directly integrated into the training of the prediction network, demonstrating favorable effectiveness to learn from noisy labels.} %Experimental results demonstrate that our amortized meta-learning network can better fit the true distribution and achieve optimal results for multiple noise rate cases.


We conduct experiments on the CIFAR10, CIFAR100, Clothing1M, and Food-101N datasets to evaluate the proposed WarPI. The experimental results show that our method consistently outperforms the state-of-the-art method under a variant of noise ratios. Extensive analysis and study illustrate the complementary effectiveness of WarPI. 

==> 3-related.tex <==

% \textbf{Meta-learning}, or learning to learn, endues machine learning models the ability to improve their performance by leveraging knowledge extracted from a number of prior tasks. It has received increasing research interest with breakthroughs in many directions~\citep{finn2017model,rusu2018meta,gordon2018meta,rajeswaran2019meta}. Gradient-based methods (e.g., MAML~\citep{finn2017model}) learn an appropriate initialization of model parameters and adapt it to new tasks with only a few gradient steps~\citep{finn2018, zintgraf2019fast, rusu2018meta}. Learning a shared optimization algorithm has also been explored in order to quickly learn of new tasks~\citep{ravi2017optimization,andrychowicz2016learning,chen2017learning}. 

% Memory-based methods learn to leverage an external memory module to store and leverage key knowledge for quick adaptation~\citep{santoro2016meta,ramalho2019adaptive}. 
% Bayesian meta-learning methods~\citep{edwards2016towards,finn2018probabilistic, gordon2018meta,saemundsson2018meta} usually rely on hierarchical Bayesian models to learn the shared statistical information among different tasks and reason about the uncertainty over models. 
% Differentiable solution methods~\citep{liu2018learning, bertinetto2018meta} learn a universal feature embedding and obtain a task-specific learner with a closed-form solution.









% \textbf{Metric learning} has been widely studied with great success for few-shot learning~\citep{vinyals2016matching,snell2017prototypical,satorras2018few,oreshkin2018tadam,allen2019infinite}. The basic assumption is that a common metric space is shared across related tasks. Snell et al.~\cite{snell2017prototypical} constructed a prototype for each class by averaging feature representations of samples from the class in the metric space. The query images are matched to prototypes by computing their distances to conduct classification. To enhance the prototype representation, Allen et al.~\cite{allen2019infinite} proposed an infinite mixture of prototypes (IMP) to adaptively represent data distribution of each class instead of using a single vector. In addition, Oreshkin et al.~\cite{oreshkin2018tadam} proposed task dependent adaptive metric for improved few-shot learning. They established prototypes of classes conditioning on a task representation encoded by a task embedding network.

% %Graphical neural network (GNN) based models generalize the matching methods by learning the message propagation from the support set and transferring it to the query set~\citep{garcia2018few}.

% While these meta-learning algorithms have made great progress in few-shot learning tasks, exploring prior knowledge from previous tasks remains an open challenge~\citep{titsias2019functional}. In this work, we introduce kernels based on random features as the base-learners, which enables us to acquire shared knowledge across tasks by modeling their dependency via the random feature basis of kernels.

% %\textbf{Kernel learning with random Fourier features} is a versatile and powerful tool in machine learning~\citep{bishop2006pattern, hofmann2008kernel, shervashidze2011weisfeiler}. Pioneering works~\citep{bach2004multiple,gonen2011multiple, duvenaud2013structure} learn to combine predefined kernels in a multi-kernel learning manner. Kernel approximation by random Fourier features (RFFs)~\citep{rahimi2008random} is an effective technique for efficient kernel learning~\citep{gartner2002multi}, which has recently become increasingly popular~\citep{sinha2016learning,carratino2018learning}. Recent works~\citep{wilson2013gaussian} learn kernels in the frequency domain by modeling the spectral distribution as a mixture of Gaussians and computing its optimal linear combination. Instead of modeling the spectral distribution with explicit density functions, other works focus on optimizing the random base sampling strategy~\citep{yang2015carte, sinha2016learning}. Nonetheless, it has been shown that accurate approximation of kernels does not necessarily result in high classification performance \citep{avron2016quasi,chang2017data}. This suggests that learning adaptive kernels with random features by data-driven sampling strategies \citep{sinha2016learning} can improve the performance, even with a low sampling rate compared to using universal random features \citep{avron2016quasi,chang2017data}.

% Our MetaVRF is the first work to introduce kernel learning with random features to the meta-learning framework for few-shot learning. The optimization of MetaVRF is naturally cast as a variational inference and the context inference offers a principled way to incorporate prior knowledge and achieve informative and adaptive kernels.

%In order to enhance the robustness of deep learning models with noisy labels, two strategies of sample re-weighting and loss correction are commonly adopted in existing works.


% \textbf{Meta-learning}, or learning to learn, endues machine learning models the ability to improve their performance by leveraging knowledge extracted from a number of prior tasks. It has received increasing research interest with breakthroughs in many directions~\citep{finn2017model,rusu2018meta,gordon2018meta,rajeswaran2019meta}. Gradient-based methods (e.g., MAML~\citep{finn2017model}) learn an appropriate initialization of model parameters and adapt it to new tasks with only a few gradient steps~\citep{finn2018, zintgraf2019fast, rusu2018meta}. Learning a shared optimization algorithm has also been explored in order to quickly learn of new tasks~\citep{ravi2017optimization,andrychowicz2016learning,chen2017learning}. 

% Memory-based methods learn to leverage an external memory module to store and leverage key knowledge for quick adaptation~\citep{santoro2016meta,ramalho2019adaptive}. 
% Bayesian meta-learning methods~\citep{edwards2016towards,finn2018probabilistic, gordon2018meta,saemundsson2018meta} usually rely on hierarchical Bayesian models to learn the shared statistical information among different tasks and reason about the uncertainty over models. 
% Differentiable solution methods~\citep{liu2018learning, bertinetto2018meta} learn a universal feature embedding and obtain a task-specific learner with a closed-form solution.

\subsection{Meta-learning}
\textbf{Meta-learning}, or learning to learn, leverages knowledge extracted from a series of tasks to enhance the performance of prediction models. Pioneering works~\citep{utgoff1986shift, bengio1990learning} were proposed to achieve dynamical adjustment of the inductive bias of learning algorithms. It has also made great breakthroughs in many directions recently~\citep{finn2017model,flennerhag2019meta,zhen2020learninga,xu2020metafun}. Typical meta-learning methods usually parameterize a learnable function as the meta learner, which can generate the parameters or statistics~\citep{mishra2017simple,zhen2020learninga,bertinetto2018meta} for base learners. Since the meta learner is usually constructed as a neural network and directly generates the corresponding variables, it regards as the black-box adaptation for base learners. Instead of explicitly designing a meta learner, gradient-based methods (e.g., MAML~\citep{finn2017model}) learn an appropriate initialization of model parameters by back-propagation through the operation of gradient descent and then adapt to novel tasks with only a few gradient steps~\citep{finn2018, zintgraf2019fast, rusu2018meta}. The idea of back-propagation through operation is general and applicable to variant learning problems, including supervised and reinforcement learning. Another recent direction is to distilling knowledge into a shared feature extractor by metric learning~\citep{vinyals2016matching}, which has achieved promising generalization performance on few-shot learning~\citep{fei2006one}. Other methods, such as memory-based models, learn to leverage an external memory module to write and read key knowledge for fast adaptation~\citep{zhen2020learningb}, especially in the more challenging task of deductive reasoning~\citep{ramalho2018adaptive}. 


\subsection{Learning with noisy labels}

\textbf{Sample re-weighting}. The main idea of the sample re-weighting strategy is to identify samples with corrupted labels and assign a small weight value to them, which is strongly related to cost-sensitive learning~\citep{Khan2018}. There are two interesting phenomenons for deep models.~\citep{arpit2017closer} 1) The loss for clean examples is usually smaller than those for noisy samples. 2) Modern deep models can memory the clean sample at the beginning of the training that is immune to label noise. Based on these observations, samples with the lowest current loss are selected as the clean data at each training epoch in~\citep{shen2019learning}. 
Curriculum learning methods like MentorNet~\citep{jiang2018Mentornet} are proposed to train a mentor network to select samples with smaller losses to guide the optimization of the student classification network.
To alleviate the accumulated error caused by the sample-selection bias in MentorNet,     Co-teaching~\citep{han2018co} is designed to train two separate classification networks simultaneously, and teach each other by leveraging samples of the same mini-batch selected with the peer network. It is also further improved by adding the disagreement-update step to avoid reducing to self-training MonterNet as the epoch increases~\citep{yu2019does}.
In addition to selecting clean samples, a more moderate strategy is to assign low weights to noisy samples, reducing the negative impact of noise. 
Boosting technique is employed in~\citep{miao2015rboost} that updates the weights by a manually designed re-weighting function.
A joint neural embedding network, CleanNet~\citep{lee2018cleannet}, has been introduced to reduce human supervision for label noise cleaning, that merely requires a fraction of categories verified by human experts. The knowledge of label noise can be then transferred to other classes.
%\citep{han2018pumpout,xinshao2019emphasis} perform a re-scaling hyper-parameter on the gradient to mitigate the guiding of samples with noisy labels.
A Bayesian probabilistic model~\citep{wang2017robust} has been designed to handle label noise that can infer the latent variables and weights from noisy data. To avoid manually designing weighting functions,
recent works adopt the idea of meta-learning that learns to generate weights from a clean meta-data set. Ren et al.~\citep{ren2018learning} sets the weights as learnable parameters and achieves a dynamic weighting strategy by the two nested loops of optimization. Furthermore, Meta-Weight-Net~\citep{shu2019meta} directly generates weights of training samples by introducing an MLP as the weighting function under the meta-learning scenario. 

% Bayesian data reweighting \citep{wang2017robust} proposed an approach that weight the 


\textbf{Loss correction} There are essentially three ways to implement the loss function correction method. (1) The basic idea is to correct the noisy label to the true one via a confusion matrix, which is calculated~\citep{sukhbaatar2015training} to restore the transformation distribution between the true label and the noisy one in the training data. By multiplying the confusion matrix to the prediction vector, the CNN classifier can effectively fit the noisy label but ensure high fidelity with the true label~\citep{tanno2019learning}. Another common strategy along this line is to correct corrupted labels with extra inference steps, including Reed~\citep{reed2014training}, Co-teaching~\citep{han2018co}, D2L~\citep{ma2018dimensionality}, S-Model~\citep{goldberger2016training}, SELFIE~\cite{song2019selfie}. Meta-data~\citep{hendrycks2018using,pereyra2017regularizing} have been also introduced for the calculation of the confusion matrix. To reduce the number of parameters in the confusion matrix, especially under the case of hundreds of categories, a masking strategy~\citep{bo2018masking} is proposed to discard invalid class transitions by incorporating a structure prior. (2) In contrast to leveraging hard labels in the learning stage, soft labels are introduced in~\citep{gao2017deep,yi2019probabilistic} that transform the one-hot label vector into a class probability distribution vector. Since the soft label has the favorable property of model uncertainty, it can be applied to data with unclear boundaries. A meta soft label corrector~\citep{yichen2020softlabel,zheng2021meta} is also designed to purify noisy labels by using meta-data. (3) Despite the effectiveness of the cross-entropy (CE) loss in supervised learning, other forms of loss functions, such as mean absolute error (MAE) have been extensively evaluated and analyzed in learning with label noise. Another idea is to resolve the overfitting of the deep network to the biased data by changing the form of the loss function. Theoretical results on noise-tolerant loss functions for binary classification are generalized to the multi-class case under sufficient conditions in~\citep{ghosh2017robust}. They claim that MAE is inherently robust to label noise compared to the cross-entropy loss. Following works~\citep{zhang2018generalized,wang2019improving} further analyze the phenomenon of poor performance of MAE with DNNs on challenging datasets, and propose a novel noise-robust loss function as a generalization of MAE and CE. Recently, an unsupervised beta mixture model~\citep{arazo2019unsupervised} on the loss value has been proposed to fit clean and noisy samples, which implements a dynamically weighted bootstrapping loss to handle noisy samples. 



\textbf{Other methods}. 
In addition to the two common strategies above, there are a number of methods to resolve label noise. The reconstruction error from an auto-encoder architecture is applied to detect outliers of noisy labels, which is optimized in a “self-paced” manner~\citep{xia2015learning}. Data augmentation, such as the mixup strategy~\citep{zhang2017mixup} can also alleviate label noise, which has been extensively studied in~\citep{Nishi_2021_CVPR}. An early-learning regularizer (ELR)~\cite{liu2020early} is proposed to prevent notorious memorization of noisy labels, based on the observation that DNNs can memorize easy samples
at the beginning, and gradually adapt to the hard as training proceeds~\cite{arpit2017closer}. The following work of robust early-learning~\citep{xia2021robust} is proposed to reduce the side
effect of forgetting clean labels in ELR. 

In contrast with existing works, our WarPI introduces a probabilistic model to learning with noisy labels under the meta-learning scenario. WarPI can model the ambiguity of the training process, which enhances the robustness of the learning algorithm. We propose to leverage the rectifying vector to correct the prediction. The rectifying vector is generated from the prediction vector and its corresponding label, thereby adding the structure information of the data and the association information between the classes.  
 

==> 4-method.tex <==

% The current problem we are solving is a classification problem with a set of weak(noisy) data examples $\{ {x_i},{y_i}\} _{i = 1}^N$ and a set of clean data $\{ {x_i},{y_i}\} _{i = 1}^M$ where N is the number of entire training data and M is much smaller than N. In order to attain the better performance by the wake labels, we construct a new network to modify loss by calibrating the probability of logits (CPL). The CPL uses the idea of meta-learning to reweight the distribution of logits and approximate the most realistic label distribution utilizing a probabilistic model. 

% The classification network $F$ aims to predict the label of input samples and $w$ denotes its parameters. The CPL is a meta model $V$ seen as a function with parameter $\theta $, it takes a pair of the logits of example and its weak label as input and attempts to get weights ${\lambda _i}$ attach to logits ${g_i} = F({x_i};w)$. Meanwhile parameters optimization is performed in an iterative operation between the two networks. In the following, we give the derivation of the equation for parameters update.


% \textbf{CPL:} It's a MLP network with only one hidden layer. This meta-network allows the class predictions derived from classification network to be given a new distribution. The input of this network is a one-dimensional vector made up of logits and the one-hot form of label. Each hidden node is with ReLU activation function, and the output is with the Sigmoid activation function, to guarantee each value in the output vector locate in the interval of [0, 1].\\

% \subsection{Probabilistic Inference}
% CPL is not only a simple meta-learning network, we also add the part of probabilistic inference. When calculating the weights on the network for logits, what the network does is generate a latent feature space and  sample. Improving the robustness of the model by sampling and using multiple samples to approximate the true value.\\
% \\
% The posterior predictive distribution is approximated in our method as a distribution ${q_\theta }(\tilde \lambda |g,t)$. That means, we train a inference network with parameter $\theta$ that takes any training datasets' logits ${g_i}$ and its target ${t_i}$ as inputs and returns the predictive distribution over the test output ${\tilde \lambda_i}$. At the same time, we use the idea of amortizing and let an approximation ${q_\theta }(\psi |g,t)$ fit this posterior predictive distribution:
% \begin{equation}\label{}
%     {q_\theta }(\tilde \lambda |g,t){\rm{ = }}\int {p(\tilde \lambda |\psi )} {q_\theta }(\psi |g,t)d\psi 
% \end{equation}
% This step is reflected in the experiment as Monte Carlo sampling. The multiple sampling and averaging approach ensures an efficient prediction phase of the model at the test time. In the training process, we fit the true values obtained from multiple sampling from space in the form of expectations:
% \begin{equation}\label{}
%     \lambda {\rm{ =  - }}\mathbb E\limits_{p(\tilde \lambda ,g,t)} {\rm{[log }}{q_\theta }(\tilde \lambda |g,t;\theta ){\rm{] =  - }}\mathbb E\limits_{p(\tilde \lambda ,g,t)} {\rm{[log }}\int {p(\tilde \lambda |\psi ;\theta )} {q_\theta }(\psi |g,t;\theta )d\psi {\rm{]}}
% \end{equation}
% We train the weights $\lambda$ obtained in the probabilistic model together with the classification network and achieve an end-to-end training process.




% \subsection{Meta Learning process}
% The goal of optimization in common classification network is minimizing the loss $L = \frac{1}{N}\sum\limits_{i = 1}^N {l({y_i},F({x_i};w)} )$ calculated on weak dataset. Due to the presence of meta-network, we represent it in a generic way $L_i^{train} = l({y_i},F({x_i};w))$. The approach used in our function is loss-weighted. With a clean dataset and meta-network, we obtain the weights $\;{\lambda _i} = V({g_i},\;{y_i};\theta )$ attached to $i$-th sample logits. Therefore, the optimal parameter ${w^*}$ for backbone networks becomes minimizing the loss obtained after reweighting logits:
% \begin{equation}\label{}
% {w^*}(\theta ) = \mathop {arg{\mkern 1mu} {\kern 1pt} {\kern 1pt} min}\limits_w {L^{train}}(w;{\mkern 1mu} {\kern 1pt} {\kern 1pt} \theta ) \buildrel \Delta \over = \frac{1}{N}\sum\limits_{i = 1}^N {L_i^{train}(w;\theta } )
% \end{equation}
% where $ L_i^{train}(w;\theta ) = l({y_i},{V_i}(y{}_i,{g_i}(w);\theta ) \cdot {g_i}(w)) $ represents the loss function on training data.

% The parameters in CPL are updated using a clean and unbiased meta-sets, it's the meta learning idea. In our function, we use a small-scale data which guarantees correct label and data balance. The optimal parameter ${\theta ^*}$ can be obtained by iteratively running meta-data and weak data: 
% \begin{equation}\label{}
% {\theta ^*} = \mathop {\arg \min }\limits_\theta  {L^{meta}}({w^*}(\theta )) \buildrel \Delta \over = \frac{1}{M}\sum\limits_{i = 1}^M {L_i^{meta}} ({w^*}(\theta ))
% \end{equation}
% where $ L_i^{meta}(w;\theta ) = l({y_i},{V_i}(y{}_i,{g_i}(w);\theta ) \cdot {g_i}(w)) $ represents the loss function on meta data.\\
% \\
% \textbf{Training Method:} calculate the optimal parameters ${w^*}$ and ${\theta ^*}$, we refer to training approach of MAML and use an online strategy to optimize a single network.
% \\
% \textbf{*****:} Similar to a normal classification task, we select a mini-batch of training samples $\{ (x_i^{train},y_i^{train}),1 \le i \le n\} $ where 
% $n$ is the mini-batch size, and we use stochastic gradient descent (SGD) to update the parameters of the classification network. On the mini-batch data, we let the current  ${w^{(t)}}$ be trained along the direction of the optimal objective in Eq. (1):
% \begin{equation}\label{}
% \mathop {{w^{(t)}}}\limits^ \wedge  (\theta ) = {w^{(t)}} - \alpha \frac{1}{n}\sum\limits_{i = 1}^n {{\nabla _w}L_i^{train}({g_i}({w^{(t)}}) \cdot V({g_i}({w^{(t)}}),{y_i};\theta ))} {|_{{w^{(t)}}}}
% \end{equation}
% where $\alpha$ stands for step size.\\
% \textbf{Update parameters of CPL:} After Eq. (3), we obtain the updated parameters ${{w^{(t)}}}\limits^ \wedge  (\theta )$ on current batch training set. Meanwhile, we select $\{ (x_i^{meta},y_i^{meta}),1 \le i \le n\} $ from clean data. The parameter $\theta$ of CPL can be updated by Eq. (2), moving ${\theta ^{(t)}}$ along the objective gradient of Eq. (2) on the clean data:
% \begin{equation}\label{}
% {\theta ^{(t + 1)}} = {\theta ^{(t)}} - \beta \frac{1}{m}\sum\limits_{i = 1}^m {{\nabla _\theta }} L_i^{meta}(\mathop {{w^{(t)}}}\limits^ \wedge  (\theta )){|_{{\theta ^{(t)}}}}
% \end{equation}
% where $\beta$ stands for step size.\\
% \textbf{Update parameters of classifier network:}Let the updated ${\theta ^{(t + 1)}}$   participate in the update of the classification network parameter $w$:
% \begin{equation}\label{}
% {w^{(t{\rm{ + }}1)}} = {w^{(t)}}{\rm{ - }}\alpha \frac{1}{n}\sum\limits_{i = 1}^n {{\nabla _w}L_i^{train}({g_i}({w^{(t)}}) \cdot V({g_i}({w^{(t)}}),{y_i};{\theta ^{(t + 1)}}))} {|_{{w^{(t)}}}}
% \end{equation}

% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{lrrrrr}
%     \toprule
%     \multicolumn{6}{l}{\textbf{Algorithm 1} The CPL Learning Algorithm} \\
%     \midrule
%     \multicolumn{6}{l}{\textbf{Input}: Training data $D$, meta-data $\hat{D}$, batch size $n, m$ max iterations $T$} \\
%     \multicolumn{6}{l}{\textbf{Output}: Classifier network parameter $w^{(T)}$} \\
%     \multicolumn{6}{l}{1: Initialize classifier network parameters $W^{(0)}$ and CPL parameters $\theta^{(0)}$} \\
%     \multicolumn{6}{l}{2: for $t$=0 to $T$-1 do} \\
%     \multicolumn{6}{l}{3:\quad \quad
% ${x^{train}},\;{y^{train}}\; \leftarrow \;SampleMiniBatch(D,\;\;n).$ } \\
%     \multicolumn{6}{l}{4:\quad \quad
% ${x^{meta}},\;{y^{meta}}\; \leftarrow \;SampleMiniBatch(\hat D,\;\;m).$} \\
%     \multicolumn{6}{l}{5:\quad \quad    Formulate the classifier learning function 
% ${\hat w^{\left( t \right)}}\left( \theta  \right),\;\;{\nabla _w}L({w^{(t)}};{\theta ^{(t)}})$ by Eq. (3)} \\
%     \multicolumn{6}{l}{6:\quad \quad    Update 
% ${\theta ^{\left( {t + 1} \right)}},\;{\nabla _\theta }L({w^{(t)}};{\theta ^{(t)}})$ by Eq. (4)} \\
%     \multicolumn{6}{l}{7:\quad \quad    Update 
% ${w ^{\left( {t + 1} \right)}},\;{\nabla _\theta }L({w^{(t)}};{\theta ^{(t+1)}})$ by Eq. (5)} \\
%     \multicolumn{6}{l}{8: end for} \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%

We propose to learn to rectify the training processing within the meta-learning scenario. A meta-network generates a rectifying vector, which promotes robust learning with noisy labels. By treating the rectifying vector as a latent variable, the learning procedure can be formulated as a hierarchical probabilistic model. Varied from deterministic models, we introduce an amortized meta-network to estimate the distribution of the rectifying vector to enhance its robustness.

\subsection{Learning with meta-data}
In addition to the noisy training set $D_N = \{\mathbf{x}^i,\mathbf{y}^i\} _{i = 1}^N$ with $N$ samples, we provide a smaller set of clean samples $D_M = \{ \tilde{\mathbf{x}}^i,\tilde{\mathbf{y}}^i\} _{i = 1}^M$, referred to as the meta-data set, under the setting of meta-learning, where $N \gg M$. Differed with conventional supervised learning, there exists an extra meta-network $V(\mathbf{y}^i, \mathbf{z}^i; \phi )$ with the parameter of $\phi$ that takes logits $\mathbf{z}^i$ of the sample and its corresponding label $\mathbf{y}^i$ as input. The output of the meta-network is a vector $\mathbf{v}^i$ for the current sample $(\mathbf{x}^i,\mathbf{y}^i)$ that rectifies the learning process of the classifier. Given the rectifying vector $\mathbf{v}^i$, the classification network $F(\mathbf{x}^i, \mathbf{v}^i;\theta)$ with the parameter of $\theta$ can achieve robustness learning on the main task of classification with corrupted labels by multiplying $\mathbf{v}^i$ on the logits. %The two networks are jointly trained 

%The current problem we are solving is a classification problem with a set of weak(noisy) data examples $\{ {x_i},{y_i}\} _{i = 1}^N$ and a set of clean data $\{ {x_i},{y_i}\} _{i = 1}^M$ where N is the number of entire training data and M is much smaller than N. In order to attain the better performance by label noise, we construct a method with warped probabilistic inference (WarPI) to keep our model free from label noise. The WarPI uses the idea of meta-learning and probabilistic inference, which obtains a vector that we call it the warp of logits by learning the information from logits and label in meta-network. Besides, the warped vector generated by meta-network we model it as a latent variable and make it integrated into the classification network after sampling.


\subsection{Warped Probabilistic Inference}
To enhance the robustness of the model, we propose to formulate the inference process as a hierarchical probabilistic model, warped probabilistic inference (WarPI). Unlike those methods that correct the corrupted label to the pseudo one, our model meta-learns a warp $\mathbf{v}$ for the loss surface of the classification network to produce effective update direction under the case of noisy labels.   
Here, we consider the rectifying vector $\mathbf{v}$ as a latent variable. The goal of our task is to meta-learn accurate approximations to the posterior predictive distribution with shared parameters $\theta$
\begin{equation}\label{eq:ppd}
\mathcolorbox{yellow}{
	p(\mathbf{y}|\mathbf{x}, \theta)  = \int p(\mathbf{y}| \mathbf{x},\mathbf{v}, \theta)p(\mathbf{v}| \mathbf{x}, \theta)\text{d}\mathbf{v}.}
\end{equation}


The rectified learning process comprises two steps. First, form the posterior distribution \hl{$p(\mathbf{v}| \mathbf{x},\theta)$} over $\mathbf{v}$ for each sample. Second, compute the posterior predictive $p(\mathbf{y} | \mathbf{x}, \mathbf{v}, \theta)$. Since the posterior is intractable, we approximates the posterior predictive distribution in Eq. (\ref{eq:ppd}) by an amortized distribution 
\begin{equation}\label{eq:ad}
q_\phi(\mathbf{y} | \mathbf{x}) = \int p(\mathbf{y} | \mathbf{x}, \mathbf{v})q_\phi(\mathbf{v}| \mathbf{x},\mathbf{y})\text{d}\mathbf{v}. 
\end{equation}
Specifically, we construct an amortized distribution $q_\phi(\mathbf{v}| \mathbf{x},\mathbf{y})$ by introducing the meta-network $\phi$ that takes $(\mathbf{x},\mathbf{y})$ as inputs and returns the distribution over the rectifying vector $\mathbf{v}$. In our work, we choose the factorized Gaussian distribution for $q_\phi(\mathbf{v}| \mathbf{x},\mathbf{y})$ where the mean and variance are computed from the meta-network $\phi$. The graphical model corresponding to our framework is illustrated in Figure \ref{fig:prob}. 

\begin{figure}  
\centering  
\includegraphics[width=9cm]{figs/probabilistic.pdf}  
\caption{The probabilistic graphical model of the WarPI. The dashed lines denotes the inference operation for approximation ${q_\phi }(\mathbf{v}|\mathbf{x},\mathbf{y})$, while the solid lines denotes the conditional generative model $p_\theta(\mathbf{y}|\mathbf{x},\mathbf{v})$.}
\label{fig:prob}  
\end{figure} 

To evaluate the quality of the approximation of the predictive posterior, we choose the KL-divergence between the true predictive posterior and the approximated one $\KL[p(\mathbf{y}|\mathbf{x}) || q_\phi(\mathbf{y} | \mathbf{x})]$. The goal of learning is to minimize the expectation of the KL value over samples
\begin{equation}\label{eq:kl}
\phi^* =  \mathop{\argmin}_{\phi}  \mathop{\E}_{p(\mathbf{x})}  [\KL[p(\mathbf{y}|\mathbf{x}) || q_\phi(\mathbf{y} | \mathbf{x})]].
\end{equation}
The training process will finally return the amortizing network $\phi$ that best approximates the posterior predictive distribution. Indeed, the optimal will recover the true posterior $p(\mathbf{v}| \mathbf{x},\mathbf{y})$ if $q_\phi(\mathbf{v}| \mathbf{x},\mathbf{y})$ in Eq. (\ref{eq:ad}) is powerful enough. The optimization in Eq. (\ref{eq:kl}) is closed related to the maximization of the log density of the predictive distribution. In this case, we have
\begin{equation}\label{eq:kl2log}
\mathop{\E}_{p(\mathbf{x})}  [\KL[p(\mathbf{y}|\mathbf{x}) || q_\phi(\mathbf{y} | \mathbf{x})] + \text{H}(p(\mathbf{y} | \mathbf{x})) ] = \mathop{\E}_{p(\mathbf{x},\mathbf{y})} [-\log q_\phi(\mathbf{y} | \mathbf{x})],
\end{equation}
where $\text{H}(p)$ is the entropy of $p$. Thus, we derive the tractable objective function
\begin{equation}\label{eq:log}
\mathop{\argmax}_{\phi} \mathop{\E}_{p(\mathbf{x},\mathbf{y})} \log \int p_\theta(\mathbf{y} | \mathbf{x}, \mathbf{v})q_\phi(\mathbf{v}| \mathbf{x},\mathbf{y})\text{d}\mathbf{v}.
\end{equation}



%Therefore, the learned approximate inference 


%WarPI is not only a simple meta-learning network, we also add the part of probabilistic inference.~\citep{grant2018recasting}. When calculating the weights on the network for logits, what the network does is generate a latent feature space and  sampling. Improving the robustness of the model by sampling and using multiple samples to approximate the true value.

 

\iffalse
The posterior predictive distribution is approximated in our method as a distribution ${q_\theta }(z|x,y)$. That means, we train a inference network with parameter $\theta$ that takes any training datasets' logits ${x_i}$ and its target ${y_i}$ as inputs and returns the predictive distribution over the test output ${z_i}$. At the same time, we use the idea of amortizing and let an approximation ${p _\phi }(y|x,z)$ fit this posterior predictive distribution:
\begin{equation}\label{}
\begin{split}
p(y|x) & = {\int p _\phi }(y|x,z){q_\theta }(z|x,y)dz\\
% &= E_{{q_\theta }(z|x,y)}[p_\phi (y|x,z)]
\end{split}
\end{equation}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The Eq. (\ref{eq:log}) indicates the inference procedure: (i) randomly select a sample $(\mathbf{x}_i, \mathbf{y}_i)$; (ii) form the posterior predictive distribution $q(\mathbf{y}_i|\mathbf{x}_i)$ based on Eq. (\ref{eq:ad}); (iii) calculate the log-likelihood $q_\phi(\mathbf{y}_i | \mathbf{x}_i)$. Indeed, this framework is generalized from the Bayesian decision theory (BDT) \citep{gordon2018metalearning}. The optimal prediction in BDT minimizes the expected distributional loss with predictive distribution $q(\mathbf{y}|\mathbf{x})$ over the variable $\mathbf{y}$
%{\color{red} ??????}
\begin{equation}\label{eq:bdt}
\mathop{\argmin}_{q} \int p(\mathbf{y} | \mathbf{x})L(\mathbf{y} ,q(\cdot)) \text{d}\mathbf{y},
\end{equation}
where $p(\mathbf{y} | \mathbf{x}) = \int p(\mathbf{y}  | \mathbf{x}, \mathbf{v}) p(\mathbf{v}  | \mathbf{x}) \text{d}\mathbf{v} $ is the Bayesian predictive distribution and \hl{$L(\mathbf{y}, q(\cdot))$ denotes the cost between the true label $\mathbf{y}$ and prediction $q(\mathbf{y}|\mathbf{x})$ which is omitted as $q(\cdot)$.}

In practice, we implement the amortizing meta-network $V$ with parameters $\phi$ that takes a pair of the logits of the observation and label as input and outputs the distribution of the rectifying vector $q$. By sampling a rectifying vector $\mathbf{v}$ from $q$, the classification network $F$ with parameters $\theta$ get a rectified prediction $\hat{\mathbf{y}}$ with $\mathbf{v}$. We can get an unbiased estimate of the objective in Eq. (\ref{eq:log}) via Monte Carlo Sampling of repeating the above process many times and averaging results.    % from the  of input samples and $w$ denotes its parameters.   The classification network $F$ aims to predict the label of input samples and $w$ denotes its parameters. The WarPI is a meta model $V$ seen as a function with parameter $\theta $, it takes a pair of the logits of example and its weak label as input and attempts to get vector ${v _i}$ attach to logits ${f_i} = F({x_i};w)$. 



%\textbf{WarPI:} It's a MLP network with only one hidden layer. The input of this network is a one-dimensional vector made up of logits and the one-hot form of label. Each hidden node is with ReLU activation function, and the output is with the Sigmoid activation function, to guarantee each value in the output vector locate in the interval of [0, 1].\\



%A generalization of the new inference framework presented in Section 2 is based upon Bayesian decision theory (BDT). BDT provides a recipe for making predictions y for an unknown test variable y by combining information from observed training data D(t) (here from a single task t) and a loss function L(y, y) that encodes the cost of predicting y when the true value is y(Berger, 2013; Jaynes, 2003). In BDT an optimal prediction minimizes the expected loss (suppressing dependencies on the inputs and  to reduce notational clutter)

% The expected reconstruction error obtained from Eq.(1) needs to be estimated by sampling. we use Monte Carlo Sampling Methods to estimate the function $p (y|x,z)$.
% \begin{equation}\label{}
%  E_{{p_\theta }(z|x,y)}[p_\phi(y_i|x_i)] =\frac{1}{L} \sum_{l=1}^{L} p_\phi (y_i|x_i,z_i^{l})  \qquad with\quad  z_i^{l}\sim{q_\theta }(z|x_i,y_i)
% \end{equation}
% Since this expectation needs is used as part of the loss function for the parameters updating by stochastic gradient descent method, sampling $ z_i^{l} $ from ${q_\theta }(z|x_i,y_i)$ will result in the inability of gradient calculation. Thus we use the reparameterization proposed in VAE ~\citep{kingma2013auto}.
% \begin{equation}\label{}
% z_i^{l}=g(\epsilon_i^{l},x_i,y_i)\qquad with \quad \epsilon^{l}\sim p(\epsilon)
% \end{equation}
% More specifically, since we assume that the hidden variable z obeys the Gaussian distribution\\ $z_i\sim N(\mu_i ,\sigma^2_i)$, $z_i$ is then calculated by $z_i=\mu_i+\sigma  _i\cdot\epsilon _i$ with $\epsilon _i\sim N(0 ,1)$. In this way, the output of meta-learner ($\mu$ and $\sigma$) can be written in the loss function to participate in the back-propagation of the gradient.

% Next, We construct the expected results for the full traning data set in the minibatch form. Where the training set $D^{train}\{x_i,y_i\}_{i}^N$ contains a total of N samples, and each minibatch $D^{m}\{x_i,y_i\}_{i}^M$ is a random sample of M samples drawn from the total training set.
% \begin{equation}\label{}
%  L^{train} \approx \frac{N}{M}\sum_{i=1}^{M}\frac{1}{L} \sum_{l=1}^{L} p_\phi (y_i|x_i,z_i^{l}) 
% \end{equation}
% Theoretically, the number of samples L should be large enough to ensure the accuracy of the results. However, experiments have shown that when the value of M is large enough, a smaller value of L is sufficient to obtain satisfactory results. 

% The multiple sampling and averaging approach ensures an efficient prediction phase of the model at the test time.~\citep{edwards2016towards} In the training process, we fit the true values obtained from multiple sampling from space in the form of expectations.

% \begin{figure}  
% \centering  
% \includegraphics[height=8.09cm,width=16cm]{ACML2021/figs/WarPI_.pdf}  
% \caption{}  
% \label{1}  
% \end{figure}  

\subsection{Learning process}
There are two networks in our framework. The amortizing meta-network $V(\cdot)$ takes logits and corrupted labels of the sample as inputs to generate the distribution $q(\mathbf{v})$ of the rectifying vector $\mathbf{v}$, while the classification network $F(\cdot)$ employs the sampled $\mathbf{v}$ to estimate the predictive posterior. The optimization for two networks is conducted via a bi-level iterative updating. We provide the exhaustive derivation for each updating step in the following. 

\subsubsection{The objectives}
In order to achieve better generalization under the case of noisy labels, the objective for our prediction model $F_\theta(\cdot)$ is to minimize the rectified loss with the support of the meta-network 
\begin{equation}\label{eq:obj0}
\mathop{\argmin}_{\theta} L^{train}(\theta) = \frac{1}{N}\sum\limits_{i = 1}^N  L(\mathbf{y}^i,\mathbf{v}^i \odot F(\mathbf{x}^i;\theta)),
\end{equation}
where $\mathbf{v}^i$ is sampled from the distribution $q(\mathbf{v})$ computed by the meta-network $q^i(\mathbf{v}) \leftarrow V(F(\mathbf{x}^i;\theta)),\mathbf{y}^i, \phi)$. \hl{Note that $F(\mathbf{x}^i;\theta))$ is the output of the fully-connected layer. By multiplying $\mathbf{v}^i$ to $F(\mathbf{x}^i;\theta))$ with Hadamard product $\odot$, also known as element-wise product, we compute the cross-entropy loss with the softmax function from the rectifying logits.} More specifically, since we assume that the variable $\mathbf{v}$ obeys a factorized Gaussian distribution $\mathbf{v}\sim N(\mu ,\sigma^2)$, we adopt the reparameterization trick proposed in~\citep{kingma2013auto} to perform back-propagation of the sampling operation as
\begin{equation}\label{eq:reparam}
\mathbf{v}=\mu + \sigma \cdot \epsilon \quad \text{with} \;\; \epsilon \sim \mathcal{N}(0 ,\text{I}).
\end{equation}
Here, $(\mu, \sigma)$ are the output of the meta-network. We denote $\text{RP}$ as the sampling operation with the reparameterization trick in the following section. 

\textbf{The objective for $\theta$}. Recall the aim of computing the predictive posterior. We attain its unbiased estimation via Monte Carlo sampling. Supposing $\mathbf{v}$ are sampled $\ell$ times, the objective in Eq. (\ref{eq:obj0}) can be rewritten as 
\begin{equation}\label{eq:obj1}
\mathop{\argmin}_{\theta} \, L^{train}(\theta) = \frac{1}{\ell N}\sum\limits_{i = 1}^N \sum\limits_{j = 1}^\ell L(\mathbf{y}^i, \text{RP}^{(j)}[V(F(\mathbf{x}^i;\theta), \mathbf{y}^i; \phi )] \odot F(\mathbf{x}^i;\theta)).
\end{equation}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% comments %%%%%%%%%%%%%%%%%%%%%
\iffalse
The goal of optimization in common classification network is minimizing the loss $L = \frac{1}{N}\sum\limits_{i = 1}^N {l({y_i},F({x_i};w)} )$ calculated on training dataset with noise. Due to the presence of meta-network, we represent it in a generic way $L_i^{train} = l({y_i},F({x_i};w))$. The approach used in our function is loss-weighted. With a clean dataset and meta-network, we obtain the weights $v = V({y_i},F({x_i};w)\;\theta )$ attached to $i$-th sample logits. Therefore, the optimal parameter ${w^*}$ for backbone networks becomes minimizing the loss obtained after reweighting logits:
\begin{equation}\label{}
{w^*}(\theta ) = \mathop {arg{\mkern 1mu} {\kern 1pt} {\kern 1pt} min}\limits_w {L^{train}}(w;{\mkern 1mu} {\kern 1pt} {\kern 1pt} \theta ) \buildrel \Delta \over = \frac{1}{N}\sum\limits_{i = 1}^N {L_i^{train}(w;\theta } )
\end{equation}
where $ L_i^{train}(w;\theta ) = l({y_i},{V_i}(y{}_i,F({x_i};w);\theta ) \odot  F({x_i};w)) $ represents the loss function on training data. Based on the probability model, the negative value of log likelihood can be written as:

\begin{equation}\label{}
\begin{split}
-log\ p(y|x) & = {\int -log\ p _\phi }(y|x,z){q_\theta }(z|x,y)dz\\
&= E_{{q_\theta }(z|x,y)}[-log\ p_\phi (y|x,z)]
\end{split}
\end{equation}


The expected reconstruction error obtained from Eq.(1) needs to be estimated by sampling. we use Monte Carlo Sampling Methods to estimate the function $p (y|x,z)$.
\begin{equation}\label{}
 E_{{p_\theta }(z|x,y)}[-log\ p_\phi(y_i|x_i)] =\frac{1}{L} \sum_{l=1}^{L} -log\ p_\phi (y_i|x_i,z_i^{l})  \qquad with\quad  z_i^{l}\sim{q_\theta }(z|x_i,y_i)
\end{equation}
Since this expectation needs is used as part of the loss function for the parameters updating by stochastic gradient descent method, sampling $ z_i^{l} $ from ${q_\theta }(z|x_i,y_i)$ will result in the inability of gradient calculation. 

Thus we use the reparameterization proposed in VAE ~\citep{kingma2013auto}.
\begin{equation}\label{}
z_i^{l}=g(\epsilon_i^{l},x_i,y_i)\qquad with \quad \epsilon^{l}\sim p(\epsilon)
\end{equation}
More specifically, since we assume that the hidden variable z obeys the Gaussian distribution $z_i\sim N(\mu_i ,\sigma^2_i)$, $z_i$ is then calculated by $z_i=\mu_i+\sigma  _i\cdot\epsilon _i$ with $\epsilon _i\sim N(0 ,1)$. In this way, the output of meta-learner ($\mu$ and $\sigma$) can be written in the loss function to participate in the back-propagation of the gradient.

Next, We construct the expected results for the full trianing data set in the minibatch form. Where the training set $D^{train}\{x_i,y_i\}_{i}^N$ contains a total of N samples, and each minibatch $D^{m}\{x_i,y_i\}_{i}^M$ is a random sample of M samples drawn from the total training set.
\begin{equation}\label{}
 L^{train} \approx \frac{N}{M}\sum_{i=1}^{M}\frac{1}{L} \sum_{l=1}^{L} -log\ p_\phi (y_i|x_i,z_i^{l}) 
\end{equation}
Regarding as the selection of the value L, we conduct further analysis in the Section Experiments. 
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% comments end %%%%%%%%%%%%%%%%%%%%%

The Monte Carlo sampling and averaging strategies for estimating the posterior ensure an efficient feed-forward propagation phase of the model at the training time. We have conducted further analysis of balancing their efficiency and accuracy in experiments. %In the training process, we fit the true values obtained from multiple sampling from space in the form of expectations.

\textbf{The objective for $\phi$}. Besides, the meta-network in WarPI is also evaluated by using a clean unbiased meta-data set $D_M$. Note that the updated $\theta$ is closely corresponding to $\phi$. Once we obtain $F(\cdot)$ with parameters $\theta^*(\phi)$, the objective for the meta-network is
\begin{equation}\label{eq:obj2}
\begin{split}
\mathop{\argmin}_{\phi} \, L^{meta}(\phi) = \frac{1}{M}\sum\limits_{i = 1}^M  L(\tilde{\mathbf{y}}^i, F(\tilde{\mathbf{x}}^i;\theta^*(\phi))).
\end{split}
\end{equation}
By minimizing Eq. (\ref{eq:obj2}) with respect of $\phi$, the learned $V_{\phi^*}$ can 
generate effective rectifying vectors to guide following updates for $F_{\theta}$.


\iffalse
The parameters in WarPI are updated using a clean and unbiased meta-sets, it's the meta learning idea. In our function, we use a small-scale data which guarantees correct label and data balance. The optimal parameter ${\theta ^*}$ can be obtained by iteratively running meta-data and weak data: 
\begin{equation}\label{}
{\theta ^*} = \mathop {\arg \min }\limits_\theta  L^{meta}({w^*}(\theta )) \buildrel \Delta \over = \frac{1}{M}\sum\limits_{i = 1}^M {L_i^{meta}} ({w^*}(\theta ))
\end{equation}
where $ L_i^{meta}(w;\theta ) = l({y_i},{V_i}(y{}_i,F({x_i};w);\theta ) \odot  F({x_i};w)) $ represents the loss function on meta data.
\fi

\begin{figure}  
\centering  
\includegraphics[width=8.5cm]{figs/flowchart.pdf}  
\caption{Flowchart of our WarPI learning algorithm \ref{alg:1}. The solid and dashed lines denote forward and backward propagation, respectively. The meta-network $V_\phi$ generates the distribution of the rectifying vector $\mathbf{v}$, and then produces multiple examples via the sampling module. By backpropagating through the updating process of step 4, the meta-network can be optimized with step 5. The classification network will be optimized with support of the learned meta-network thereafter.}
\label{fig:flowchart}  
\end{figure}  




\subsubsection{Iterative optimization} 
To calculate the optimal parameters ${\theta^*}$ and ${\phi^*}$, we resort to a bi-level iterative optimization as MAML~\citep{finn2017model} and use an online strategy to optimize the meta-network.


\textbf{Learning process for $F_\theta(\cdot)$}. For each iterative step of the classification network, we sample a mini-batch of $n$ training examples $\{(\mathbf{x}^i,\mathbf{y}^i) \}^n_{i=1}$. The updating step with the size of $\alpha$ for $F_\theta(\cdot)$ \textit{w.r.t.} Eq. (\ref{eq:obj1}) can be derived as
\begin{equation}\label{eq:theta_step}
\hat{\theta}^{(t)}(\phi )  = \theta^{(t)} - \alpha \frac{1}{\ell n}\sum\limits_{i = 1}^n \sum\limits_{j = 1}^\ell \nabla _\theta L(\mathbf{y}^i, \text{RP}^{(j)}[V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i; \phi )] \odot F(\mathbf{x}^i;\theta^{(t)})).
\end{equation}

\textbf{Updating $\phi$ with the learning process of $\theta$}. As we obtain parameters  $\hat{\theta}^{(t)}(\phi)$ with fixed $\phi$ in Eq. (\ref{eq:theta_step}), \hl{the meta-network $V_\phi(\cdot)$ can be updated by using a batch of $m$ meta samples $\{(\tilde{\mathbf{x}}^i,\tilde{\mathbf{y}}^i) \}^m_{i=1}$.} Specifically, ${\phi^{(t)}}$ moves along the direction of gradients \textit{w.r.t.} the objective in Eq. (\ref{eq:obj2})
\begin{equation}\label{eq:phi_update}
\mathcolorbox{yellow}{
\phi^{(t + 1)} = {\phi^{(t)}} - \beta \frac{1}{m}\sum\limits_{i = 1}^m {{\nabla _\phi }} L(\tilde{\mathbf{y}}^i, F(\tilde{\mathbf{x}}^i;\hat{\theta}^{(t)}(\phi^{(t)}))),}
\end{equation}
where $\beta$ denotes the step size. Typically, the gradient-based update rule for $\phi$ is to compute gradients through the learning process of $\theta$, which is similar as MAML.

\textbf{Update $\theta$ with the learned $\phi$}. We employ the updated $V_{\phi^{(t + 1)}}(\cdot)$ to improve learning of the classification network $F_{\theta}(\cdot)$
\begin{equation}\label{eq:theta_update}
\theta^{(t+1)} = \theta^{(t)}- \alpha \frac{1}{\ell n}\sum\limits_{i = 1}^n \sum\limits_{j = 1}^\ell \nabla _\theta L(\mathbf{y}^i, \text{RP}^{(j)}[V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i; \phi^{(t+1)} )] \odot F(\mathbf{x}^i;\theta^{(t)})).
\end{equation}

The overall steps can be summarized in Algorithm \ref{alg:1}. The main steps are illustrated in Figure \ref{fig:flowchart}. Thanks to the reparameterization trick, the sampling operation can be implemented as a linear transformation, which is tractable for gradient computation. Besides, estimating predictive posterior in Eq. (\ref{eq:obj1}) by Monte Carlo sampling of averaging $\ell$ results can be also efficient. All gradients computations, including those in the bi-level iterative process, can be efficiently implemented by automatic differentiation tools.   
%The probability model is not explicitly shown in the learning process because it is included in the meta-learner. the distribution of warp vector (hidden variables z) is obtained by the last layer of meta-network, and then sample L times to calculate a set of warped vector, multiply them separately with the logits obtained from the classifier and the average is the warped prediction vector $ \tilde {y}$, which is closed to noisy label. 


\begin{algorithm}[t]
\caption{The WarPI Learning Algorithm}
\label{alg:1}
\begin{algorithmic}[1]
\REQUIRE 
Training data $D_N$, meta data $D_M$    \hfill $\triangleright$ Datasets \\
Batch size $n, m$, outer iterations $T$,%, inner iterations $K$
\\  sample number $\ell$, learning rate $\alpha$, $\beta$		\hfill $\triangleright$ Hyper-parameters
\\
\ENSURE Optimal $\theta^*$ \\
\STATE  Initialize parameters $\theta^{(0)}$ and $\phi^{(0)}$ \\
\FOR{$t \in \{1,\dots,T\}$}
        \STATE $(\mathbf{x}, \mathbf{y}), (\tilde{\mathbf{x}}, \tilde{\mathbf{y}})\leftarrow \text{SampleBatch}(D_N, n), \text{SampleBatch}(D_M, m)$\\
        \STATE Formulate learning process of $\theta$ with probabilistic inference \hfill $\triangleright$ Eq. (\ref{eq:theta_step}) \\
        \STATE Update $\phi$ with the learning process of $\theta$ \hfill $\triangleright$ Eq. (\ref{eq:phi_update}) \\ 
        \STATE Update $\theta$ with the learned $\phi$ \hfill $\triangleright$ Eq. (\ref{eq:theta_update}) \\ 
\ENDFOR \\
\end{algorithmic}
\end{algorithm}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% comments
\iffalse
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
    \begin{tabular}{lrrrrr}
    \toprule
    \multicolumn{6}{l}{\textbf{Algorithm 1} The WarPI Learning Algorithm} \\
    \midrule
    \multicolumn{6}{l}{\textbf{Input}: Training data $D$, meta-data $\hat{D}$, batch size $n, m$ max iterations $T$} \\
    \multicolumn{6}{l}{\textbf{Output}: Classifier network parameter $w^{(T)}$} \\
    \multicolumn{6}{l}{1: Initialize classifier network parameters $W^{(0)}$ and WarPI parameters $\theta^{(0)}$} \\
    \multicolumn{6}{l}{2: for $t$=0 to $T$-1 do} \\
    \multicolumn{6}{l}{3:\quad \quad
${x^{train}},\;{y^{train}}\; \leftarrow \;SampleMiniBatch(D,\;\;n).$ } \\
    \multicolumn{6}{l}{4:\quad \quad
${x^{meta}},\;{y^{meta}}\; \leftarrow \;SampleMiniBatch(\hat D,\;\;m).$} \\
    \multicolumn{6}{l}{5:\quad \quad    Formulate the classifier learning function 
${\hat w^{\left( t \right)}}\left( \theta  \right),\;\;{\nabla _w}L({w^{(t)}};{\theta ^{(t)}})$ by Eq. (4)} \\
    \multicolumn{6}{l}{6:\quad \quad    Update 
${\theta ^{\left( {t + 1} \right)}},\;{\nabla _\theta }L({w^{(t)}};{\theta ^{(t)}})$ by Eq. (5)} \\
    \multicolumn{6}{l}{7:\quad \quad    Update 
${w ^{\left( {t + 1} \right)}},\;{\nabla _\theta }L({w^{(t)}};{\theta ^{(t+1)}})$ by Eq. (6)} \\
    \multicolumn{6}{l}{8: end for} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% end %%%%%%%%%%%

\subsection{Analysis of the rectification manner}
To demonstrate the property of WarPI and illustrate its effectiveness of the rectification process, we expand the updating steps of $\theta$ and $\phi$ in Eq.(\ref{eq:theta_step}-\ref{eq:phi_update}). The sampling operation of the probabilistic inference is not included in following derivation for convenience. Here, $V(F(\mathbf{x}^i;{\theta^{(t)}});\phi)$ denotes one of the sampled rectifying vector $\mathbf{v}$ in the following equation. To facilitate the further derivation we expand Eq. (\ref{eq:theta_step}) for step $t$ as
\begin{equation}\label{eq:theta_step_exp}
\begin{split}
% \frac{\partial \hat{\theta}^{(t)}(\phi)}{\partial \phi} & =\frac{\partial \theta^{(t)}}{\partial \theta \partial \phi} - \alpha \frac{1}{n}\sum\limits_{i = 1}^n \frac{\partial \left( L(F(\mathbf{x}^i;\theta^{(t)}) \odot V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )\right)}{\partial \theta \partial \phi}\\
% &= = -\alpha \frac{1}{n}\sum\limits_{i=1}^n\frac{\partial }{\partial \phi }  \left({\frac{\partial \mathbf{\hat {y}}}{\partial \theta}}^{T}\cdot \frac{\partial L(\mathbf{y}^i,\mathbf{\hat {y}})}{\partial \mathbf{\hat {y}}}\right)
\hat{\theta}^{(t)}(\phi) 
&=\theta^{(t)}
- \alpha \frac{1}{n}\sum\limits_{i = 1}^n 
\nabla_\theta {L(F(\mathbf{x}^i;\theta^{(t)}) \odot V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )}\\
&=\theta^{(t)} -\alpha \frac{1}{n}\sum\limits_{i=1}^n\frac{\partial F(\mathbf{x}^i;\theta^{(t)})}{\partial \theta }\odot  V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi ) \cdot  \frac{\partial L(\mathbf{y}^i,\mathbf{\hat {y}})}{\partial \mathbf{\hat {y}}}.
\end{split}
\end{equation}
Here, the prediction $\mathbf{\hat {y}} = F(\mathbf{x}^i;\theta^{(t)}) \odot V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )$.
Note that we detach the input $F(\mathbf{x}^i;\theta^{(t)})$ of $V(\cdot)$ from the computation graph, therefore, 
the gradient of $\hat{\theta}^{(t)}(\phi)$ with respect to $\phi$ can be written as
\begin{equation}\label{eq:theta_step_exp_gra}
\frac{\partial \hat{\theta}^{(t)}(\phi)}{\partial \phi} = \frac{\alpha }{n}\sum\limits_{i = 1}^n\frac{\partial  V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )}{\partial \phi }^{T}
\cdot\frac{\partial L(\mathbf{y}^i,\mathbf{\hat {y}})}{\partial \mathbf{\hat {y}}} \odot\frac{\partial  F(\mathbf{x}^i;\theta^{(t)})}{\partial \theta}
\end{equation}

By substituting Eq. (\ref{eq:theta_step_exp_gra}) into Eq. (\ref{eq:phi_update}), we have
\begin{equation}\label{eq:second-order}
\begin{split}
{\phi^{(t + 1)}} &= {\phi^{(t)}} - \beta \frac{1}{m}\sum\limits_{i = 1}^m {{\nabla _\phi }} L(\tilde{\mathbf{y}}^i, F(\tilde{\mathbf{x}}^i;\hat{\theta}(\phi))) \\
&= \phi ^{(t)}-\frac{\beta }{m}\sum_{j=1}^{m}\sum_{i=1}^{n} \frac{\partial \hat{\theta} ^{(t)}(\phi )}{\partial V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )}\\
& \cdot \frac{\partial  V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )}{\partial \phi}^{T} \cdot\frac{\partial L(\tilde {\mathbf{y}}^j,F(\tilde {\mathbf{x}}^j;\hat{\theta}^{(t)}(\phi ) ))}{\partial \hat{\theta}^{(t)}(\phi )}\\
& = \phi ^{(t)}+\frac{\beta }{m}\sum\limits_{j = 1}^m\frac{\alpha }{n}\sum\limits_{i = 1}^n\frac{\partial  V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )}{\partial \phi }^{T}
\cdot\frac{\partial L(\mathbf{y}^i,\mathbf{\hat {y}})}{\partial \mathbf{\hat {y}}}\\
&\odot \frac{\partial  F(\mathbf{x}^i;\theta^{(t)})}{\partial \theta }
\cdot  \frac{\partial L(\tilde {\mathbf{y}}^j,F(\tilde {\mathbf{x}}^j;\hat{\theta}^{(t)}(\phi ) ))}{\partial\hat{\theta}^{(t)}(\phi)}\\
& = \phi ^{(t)}+\frac{\alpha\cdot \beta   }{m\cdot n}\sum\limits_{j = 1}^m\sum\limits_{i = 1}^n
\frac{\partial  V(F(\mathbf{x}^i;\theta^{(t)}), \mathbf{y}^i;\phi )}{\partial \phi }^{T}
\cdot\frac{\partial L(\mathbf{y}^i,\mathbf{\hat {y}})}{\partial \mathbf{\hat {y}}}\\
&\odot\frac{\partial  F(\mathbf{x}^i;\theta^{(t)})}{\partial \theta}
\cdot \frac{\partial F(\tilde {\mathbf{x}}^j;\hat{\theta}^{(t)}(\phi ) )}{\partial \hat{\theta }^{(t)}(\phi )}^{T}
\cdot\frac{\partial L(\tilde {\mathbf{y}}^j,F(\tilde {\mathbf{x}}^j;\hat{\theta}^{(t)}(\phi ) ))}{\partial F(\tilde {\mathbf{x}}^j;\hat{\theta}^{(t)}(\phi ) )}.
\end{split}
\end{equation}
It can be shown that the gradient of $\hat{\theta}^{(t)}(\phi)$ is computed in virtue of the meta batch and then backpropagates through $V(\cdot)$ using the training batch, which is similar to MAML as gradients of updating steps.

% In the expansion of $\phi^{(t+1)}$ we can see, $\frac{\partial  F_i(w)}{\partial w}\Big|_{{w^{(t)}}} \cdot \frac{F_j(\hat{w}^{(t)}(\theta ))}{\hat{w}^{(t)}(\theta )}\Big|_{{\theta }}^{T} $ denotes the multiplication of the updated gradients of the classifier under the training samples and metadata samples, for simplicity, we write it as $A$ with $ A\subset R^{c\times c}$, where c represents the number of classes in the data set. $\tilde {y}_i$ and $F(x_j^{meta};\hat{w}^{(t)} )$ are vectors that belongs to $[0,1]^{c\times 1}$, and can be expressed as $[\gamma_1,\gamma_2...\gamma_c]^T$ and $[\eta_1,\eta_2...\eta_c  ]^T$.




% Because the loss function used in the training process is the cross-entropy loss, $\frac{\partial l_i(y_i^{train},\tilde{y}_i )}{\partial \tilde{y}}$ ( the corresponding label $y_i^{train}$ is k ) can be calculated as a vector that is $-\frac{1}{\gamma_k}$ at index of k and the rest is zero, as the same, $\frac{\partial l_j(y_j^{meta},F(x^{meta};\hat{w}^{(t)} ))}{\partial F(x_j^{meta};\hat{w}^{(t)})} $ ( the corresponding label $y_j^{meta}$ is g ) can be calculated as a vector that is $-\frac{1}{\eta_g}$ at index of g and the rest is zero. As a result, $\frac{\partial l_i(y_i^{train},\tilde{y}_i )}{\partial \tilde{y}}\Big|^{T}\odot \frac{\partial  F(x_i^{train};w^{(t)})}{\partial w}\Big|_{{w^{(t)}}} \cdot \frac{\partial F(x_j^{meta};\hat{w}^{(t)} )}{\partial \hat{w}^{(t)}(\theta )} \Big|^{T}
%  \cdot\frac{\partial l_j(y_j^{meta},F(x^{meta};\hat{w}^{(t)} ))}{\partial F(x_j^{meta};\hat{w}^{(t)})}$ is computed as a vector $h \subset R^c\times 1$, which is $\frac{A_{kg}}{\gamma_k \cdot \eta_g}$ at index of k, and the rest is zero. More specifically, $\gamma_k$ denotes the probability that the wraped prediction vector of $x_i^{train}$ belongs to class k, and $\eta_g$ denotes the probability that the prediction vector of $x_j^{meta}$ belongs to class g. That means if the wraped prediction vector of training data does not match the noisy label nor the prediction vector of meta data does not match its clean label, the parameter $\theta$ will then updated more intensely. 
% From another perspective, it illustrates that the meta-learner drives prediction vectors calculated by the classifier to fit the correct label, while at the same time makes the warped prediction vectors fit the noisy labels.

==> 5-experiments.tex <==
To evaluate the performance of WarPI, we conduct experiments with variant noise conditions on four benchmarks including CIFAR-10, CIFAR100, Clothing1M. Exhaustive study and analysis demonstrate its favorable effectiveness and great efficiency for label noise in comparison to deterministic models.   


\begin{table}[]\small
\caption{\hl{Architectures of the classification network on different datasets.}}
\centering
\label{tab:network}
%\centering
\begin{tabular}{|l|c|c|c|c|}
%\toprule
\hline
 Noise Type& Uniform & Asymmetric & Instance & Open-set  \\ \hline
CIFAR-10  & WRN-28-10       & ResNet-32    & ResNet-18      & -    \\
CIFAR-100  & WRN-28-10       & ResNet-32   & ResNet-18     & -     \\
Clothing-1M & -        & -   &-     & ResNet-50        \\
Food-101N  & -        & -    &-    & ResNet-50      \\\hline
%\toprule
\end{tabular}
\end{table}


\subsection{Datasets} 
\textbf{CIFAR-10}~\citep{krizhevsky2009learning} dataset consists of 60,000 images of 10 categories. We adopt the splitting strategy in~\cite{shu2019meta} by randomly selecting 1,000 samples from the training set to construct the meta dataset. We train the classification network on the remaining 40,000 noisy samples and evaluate the model on 1,0000 testing images. 

\textbf{CIFAR-100}~\citep{krizhevsky2009learning} is more challenging than CIFAR-10 including 100 classes belonging to 20 superclasses where each category contains 600 images with the resolution of 32 $\times$ 32. Similar splitting manners as CIFAR-10 are employed. 

\textbf{Clothing1M}~\citep{xia2019anchor} is a large-scale dataset that is collected from real-world online shopping websites. It contains 1 million images of 14 categories whose labels are generated based on tags extracting from the
surrounding texts and keywords, causing huge label noise. The estimated percentage of corrupted 
labels is around 39.46\%. A portion of clean data is also included in Clothing1M, which has been divided into the training set (50k images), validation set (14k images), and test set (10k images). We select the validation set as the meta dataset and evaluate the performance on the test set. We resize all images to $256 \times 256$ as in~\citep{shu2019meta}.

\textbf{Food-101N}~\citep{lee2018cleannet} is constructed based on the taxonomy of $101$ categories in Food-101~\citep{bossard2014food}. It consists of 310k images collected from Google, Bing, Yelp, and TripAdvisor. The noise ratio for labels is around 20$\%$. We select the validation set of 3824 as the meta-data. Following the testing protocol in~\citep{lee2018cleannet, zhang2021learning}, we learn the model on the training set of 55k images and evaluate it on the testing set of the original Food-101. 

\textbf{Label noise settings}. We study four types of corrupted labels in our experiments following the same setting in~\citep{shu2019meta}. 1) \textit{Uniform noise} is constructed by independently changing the label to a random class with a certain probability $\rho$. 2) \textit{Asymmetric noise} is also known as flip noise. For each class, we randomly select a transformed class from the remaining. The label noise is formed by independently flipping the label to the transformed class with a total probability $\rho$. \hl{3) \textit{Instance-dependent (ID) noise} stems from the uncertain annotation for the ambiguous observation. Therefore, the corrupted label is close related to the input of the image. We adopt the protocol in} \citep{xia2020part} \hl{to construct the dataset with ID noise.} 4) \textit{Open-set noise} is introduced in the collection of training data, whose form is unknown. For uniform, flip, and ID noise, we evaluate the model under variant settings of noise ratios on CIFAR-10 and CIFAR-100, where $\rho=0.2\; \text{or} \; 0.6, 0.4$. For open-set noise, we conduct experiments on the large-scale real-world datasets, Clothing1M and Food-101N. %{\color{red} }


\subsection{Setup}
\textbf{Network architectures}. For the meta-network in WarPI, we implement it as a three-layer MLP with the dimension of $100$ for hidden layers. As indicated in the method section, its input is a $2d$ vector consisting of the output of the classification network and a one-hot vector of the noisy label. Here, $d$ is the dimension of the output and the one-hot label. For the architecture of the classification network, we following the setting in~\citep{ren2018learning, hendrycks2018using,shu2019meta,zhang2021learning}, summarized in Table \ref{tab:network}.


\begin{table}[]\small
\caption{Hyperparameters in our experiments on different datasets.}
\centering
\label{tab:params}
\begin{tabular}{|l|c|c|c|c|}
%\toprule
\hline
\footnotesize{\diagbox{Hyperparams}{Dataset}} & CIFAR-10 & CIFAR-100 & Clothing1M &Food101N \\ \hline
Sample Number                & 10       & 10        & 1          & 1        \\
Batch Size                   & 100      & 100       & 128        & 128      \\
Optimizer                    & SGD      & SGD       & SGD        & Adam     \\
Initial LR                   & 0.1      & 0.1       & 0.1        & 3e-4     \\
Decay Rate (LR)              & 5e-4     & 5e-4      & 5e-4       & -       \\
Epoch                        & 80       & 80        & 10         & 30       \\
Momentum                     & 0.9      & 0.9       & 0.9        & -        \\
%\toprule
\hline
\end{tabular}
\end{table}


\textbf{Hyperparameters}. We provide detailed settings of hyperparameters in Table \ref{tab:params}. These include the number of examples in Monte Carlo sampling $\ell$, batch size, optimizers, initial learning rates with decay rates, the number of epoch, and parameters of the Momentum in SGD. Note that the number of samples $\ell$ has an important impact on performance. For CIFAR-10 and CIFAR-100, we set it as $10$ to achieve high accuracy. For large-scale dataset of Clothing1M and Food101N, we choose $1$ for the efficiency of training. Exhaustive analysis for $\ell$ is conducted in the following section.


%\textbf{Experiments on Colthing1M} To verify the effectiveness of our method in a {\color{red} open-set} environment of noise label, we choose a clothing classification dataset containing roughly {40\%} data noise. We use 14k clean data as meta dataset. Following the current work~\citep{shu2019meta, ren2018learning, hendrycks2018using}, we selected ResNet-50, which was pre-trained on ImageNet, as the classification network. The images were resized $224 \times 224$  as model input. We chose SGD as optimization function for classification network, its’ initial learning rate is 0.01, momentum is 0.9, weight decay is ${1e^{ - 3}}$. The learning rate is divided by 10 after 5 epoch(the whole epoch is 10). The batch size sets to 128 and the learning rate of WarPI is fixed as ${10^{ - 3}}$.


\begin{table}[]%\small
\centering
   \caption{Testing Acc.(\%) on CIFAR-10 and CIFAR-100 with varying ratios of uniform noise.}
   \label{tab:unif}
\begin{tabular}{|lcccc|}
%\toprule
\hline
\textbf{Dataset}   & \multicolumn{2}{c}{\textbf{CIFAR-10}}   & \multicolumn{2}{c|}{\textbf{CIFAR-100}}                       \\  
\textbf{Noise ratio}            & \textbf{0.4}   & \textbf{0.6}        & \textbf{0.4}    & \textbf{0.6} \\ \hline\hline
\textbf{Base Model}  & 68.07 &53.12&  51.11&30.92\\
%\textbf{Focal Loss}~\citep{lin2017focal}      & \textbf{95.70} & 75.96            & 51.87      & \textbf{81.04}         & 51.19      & 27.70   \\
\textbf{Co-teaching}~\citep{han2018co}                & 74.81            & 73.06                      & 46.20            & 35.67 \\
\textbf{MentorNet}~\citep{jiang2018Mentornet}                         & 87.33         & 82.80                                         & 61.39                     & 36.87                    \\
\textbf{D2L}~\citep{ma2018dimensionality}              & 85.60            & 68.02                   & 52.10      & 41.11  \\
\textbf{DMI-NS}~\citep{chen2021robustness}    & \textbf{91.11}    & 83.46               & 66.95        & 58.35  \\\hline \hline
\textbf{Fine-tuning}                      & 80.47            & 78.75                       & 52.49              & 38.16 \\
\textbf{GLC}~\citep{hendrycks2018using}             & 88.28            & 83.49                     & 61.31             & 50.81  \\
\textbf{L2RW}~\citep{ren2018learning}                 & 86.92             & 82.24                   & 60.79       & 48.15 \\
\textbf{MWNet}~\citep{shu2019meta}                 & 89.27            & 84.07                     & 67.73             & 58.75 \\
\textbf{MLC}~\citep{wang2020training}                   & 89.20            & 84.22               & - &-  \\ 
\hline
\textbf{WarPI (Detc.)}              & 89.47          & 83.93                     & 67.16              &58.77 \\
\textbf{WarPI}                        & 89.73      &\textbf{84.44}                  & \textbf{67.90}     &\textbf{59.04}\\ \hline
% \toprule
\end{tabular}
\end{table}


\begin{table}[]%\small
\centering
 \caption{Testing Acc.(\%) on CIFAR-10 and CIFAR-100 with varying ratios of asymmetric noise.}
 \label{tab:asy}
\begin{tabular}{|lcccc|}
\hline
\textbf{Dataset}         & \multicolumn{2}{c}{\textbf{CIFAR-10}}                                   & \multicolumn{2}{c|}{\textbf{CIFAR-100}}                                          \\  
\textbf{Noise ratio}           & \textbf{0.2 }           & \textbf{0.4}       & \textbf{0.2}      & \textbf{0.4}     \\ \hline\hline
\textbf{Base Model}  & 76.83& 70.77  & 50.86 & 43.01 \\
%\textbf{Focal loss}~\citep{lin2017focal}             & 93.03          & 86.45       & 80.45             & 70.02         & 61.87             & 54.13             \\
\textbf{Co-teaching }~\citep{han2018co}                        & 82.83       & 75.41                   & 54.13             & 44.85             \\
\textbf{MentorNet}~\citep{jiang2018Mentornet}                        & 86.36         & 81.76                                        & 61.97                     & 52.66                    \\
\textbf{D2L}~\citep{ma2018dimensionality}                       & 87.66        & 83.89                                         & 63.48                     & 51.83                     \\\hline\hline
\textbf{Fine-tuning}                      & 82.47          & 74.07                           & 56.98                     & 46.37                     \\
\textbf{L2RW} ~\citep{ren2018learning}                         & 87.86      & 85.66                                         & 57.47                     & 50.98                     \\
\textbf{GLC }~\citep{hendrycks2018using}                        & 89.68       & 88.92                                         & 63.07                     & 62.22                     \\
\textbf{MWNet }~\citep{shu2019meta}                          & 90.33         & 87.54                                         & 64.22                     & 58.64                     \\
\textbf{MLC}~\citep{wang2020training}        & 90.07 & 88.97  & 64.91 & 59.96 \\ \hline 
\textbf{WarPI (Detc.)}                     & 89.83                     & 88.37                                        & 64.77                     & 59.40                     \\
\textbf{WarPI}                                 & \textbf{90.93}            & \textbf{89.87}                       & \textbf{65.52}            & \textbf{62.37}             \\
\hline
\end{tabular}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse

\begin{table}[]%\small
\centering
   \caption{Testing Acc.(\%) on CIFAR-10 and CIFAR-100 with varying ratios of uniform noise.}
   \label{tab:unif}
\begin{tabular}{|lcccccc|}
%\toprule
\hline
\textbf{Dataset}   & \multicolumn{3}{c}{\textbf{CIFAR-10}}   & \multicolumn{3}{c|}{\textbf{CIFAR-100}}                       \\  
\textbf{Noise ratio}       & \multicolumn{1}{c}{\textbf{0}}     & \textbf{0.4}   & \textbf{0.6}     & \textbf{0}    & \textbf{0.4}    & \textbf{0.6} \\ \hline\hline
\textbf{Base Model} & 95.60 & 68.07 &53.12& 79.95& 51.11&30.92\\
%\textbf{Focal Loss}~\citep{lin2017focal}      & \textbf{95.70} & 75.96            & 51.87      & \textbf{81.04}         & 51.19      & 27.70   \\
\textbf{Co-teaching}~\citep{han2018co}       & 88.67          & 74.81            & 73.06              & 61.80         & 46.20            & 35.67 \\
\textbf{MentorNet}~\citep{jiang2018Mentornet}              & 94.35             & 87.33         & 82.80                     & 73.26                     & 61.39                     & 36.87                    \\
\textbf{D2L}~\citep{ma2018dimensionality}      & 94.46          & 85.60            & 68.02             & 66.17         & 52.10      & 41.11  \\
\textbf{DMI-NS}~\citep{chen2021robustness}   &  -  & \textbf{91.11}    & 83.46              &-  & 66.95        & 58.35  \\\hline \hline
\textbf{Fine-tuning}            & \textbf{95.65}           & 80.47            & 78.75              & \textbf{80.88}         & 52.49              & 38.16 \\
\textbf{GLC}~\citep{hendrycks2018using}      & 94.30         & 88.28            & 83.49              & 73.75         & 61.31             & 50.81  \\
\textbf{L2RW}~\citep{ren2018learning}        & 92.38         & 86.92             & 82.24              & 72.99         & 60.79       & 48.15 \\
\textbf{MWNet}~\citep{shu2019meta}          & 94.52          & 89.27            & 84.07              & 78.76         & 67.73             & 58.75 \\
\textbf{MLC}~\citep{wang2020training}         & 93.67          & 89.20            & 84.22              & -  & - &-  \\ 
\hline
\textbf{WarPI (Detc.)}      & 94.70          & 89.47          & 83.93              & 77.91         & 67.16              &58.77 \\
\textbf{WarPI}                 &94.33       & 89.73      &\textbf{84.44}       &77.63           & \textbf{67.90}     &\textbf{59.04}\\ \hline
% \toprule
\end{tabular}
\end{table}


\begin{table}[]%\small
\centering
 \caption{Testing Acc.(\%) on CIFAR-10 and CIFAR-100 with varying ratios of asymmetric noise.}
 \label{tab:asy}
\begin{tabular}{|lcccccc|}
\hline
\textbf{Dataset}         & \multicolumn{3}{c}{\textbf{CIFAR-10}}                                   & \multicolumn{3}{c|}{\textbf{CIFAR-100}}                                          \\  
\textbf{Noise ratio}      & \textbf{0}       & \textbf{0.2 }           & \textbf{0.4}      & \textbf{0}    & \textbf{0.2}      & \textbf{0.4}     \\ \hline\hline
\textbf{Base Model} & 92.89 & 76.83& 70.77 & 70.50 & 50.86 & 43.01 \\
%\textbf{Focal loss}~\citep{lin2017focal}             & 93.03          & 86.45       & 80.45             & 70.02         & 61.87             & 54.13             \\
\textbf{Co-teaching }~\citep{han2018co}              & 89.87          & 82.83       & 75.41             & 63.31         & 54.13             & 44.85             \\
\textbf{MentorNet}~\citep{jiang2018Mentornet}              & 92.13             & 86.36         & 81.76                     & 70.24                     & 61.97                     & 52.66                    \\
\textbf{D2L}~\citep{ma2018dimensionality}            & 92.02           & 87.66        & 83.89                     & 68.11                     & 63.48                     & 51.83                     \\\hline\hline
\textbf{Fine-tuning}          & \textbf{93.23}            & 82.47          & 74.07        & 70.72                     & 56.98                     & 46.37                     \\
\textbf{L2RW} ~\citep{ren2018learning}               & 89.25           & 87.86      & 85.66                     & 64.11                     & 57.47                     & 50.98                     \\
\textbf{GLC }~\citep{hendrycks2018using}            & 91.02             & 89.68       & 88.92                     & 65.42                     & 63.07                     & 62.22                     \\
\textbf{MWNet }~\citep{shu2019meta}              & 92.04             & 90.33         & 87.54                     & 70.11                     & 64.22                     & 58.64                     \\
\textbf{MLC}~\citep{wang2020training}        & 91.87 & 90.07 & 88.97 & 70.93 & 64.91 & 59.96 \\ \hline 
\textbf{WarPI (Detc.)} & 92.37                     & 89.83                     & 88.37                     & 70.61                     & 64.77                     & 59.40                     \\
\textbf{WarPI}            & 92.39                     & \textbf{90.93}            & \textbf{89.87}            & \textbf{71.98}            & \textbf{65.52}            & \textbf{62.37}             \\
\hline
\end{tabular}
\end{table}

\fi



\subsection{Comparison experiments}
\textbf{Uniform \& Asymmetric Noise}. 
We conduct the classification experiments on two commonly-used benchmark datasets, \textit{i.e.}, CIFAR-10 and CIFAR-100 to evaluate the performance of our model. We study two types of noise with variant noise ratios. The comparison methods include Base Model (directly training the classification network on corrupted training data), Fine-tuning (fine-tuning Base Model on the meta dataset), other mainstream methods (\textit{e. g.}, Focal loss~\citep{lin2017focal} and Co-teaching~\citep{han2018co}), and meta-learning methods (\textit{e. g.}, L2RW~\citep{ren2018learning}, MWNet~\citep{shu2019meta}, MLC~\citep{wang2020training}). The setting of generating noisy data is consistent for all methods. Other works~\citep{li2019learning} with fewer fixed confusion patterns have not been included in the comparison. We split the table into two parts for a clear illustration. The bottom consists of methods using the clean meta data, while those in the top part do not need it. To illustrate the effectiveness of the probabilistic inference in our WarPI, we also implement a deterministic model, WarPI (Detc.), by removing Monte Carlo sampling and directly generating a warped rectifying vector from the meta-network. As demonstrated in Tables \ref{tab:unif} and \ref{tab:asy}, WarPI achieves superior performance on the classification task under the setting of uniform and asymmetric noise. We would like to highlight that WarPI consistently outperforms other meta-learning methods of L2RW, MWNet, and MLC in the case of variant noise ratios. Especially, compared with the homologous approach of MWNet, our method gains significant improvement of $\mathbf{3.73\%}$ on CIFAR-100 with $40\%$ asymmetric noise. Besides, WarPI shows better performance on all settings in comparison to the deterministic model which demonstrates the effectiveness of using probabilistic inference. The result also exhibits that the deterministic model outperforms MWNet in most cases indicating the superiority of leveraging structure information in our meta-network. 


\hl{\textbf{Instance-dependent Noise}. We evaluate the performance under the challenging case of ID noise. We adopt the same strategy in} \citep{xia2020part} \hl{to construct the training set with ID label noise and consistent evaluation protocol for a fair comparison. As shown in Table} \ref{tab:inst}\hl{, WarPI achieves the best generalization performance on all evaluation settings and significantly outperforms other meta-learning methods, \textit{e. g.}, it gains improvement of $\mathbf{2.46\%}$ on CIFAR-10 with $40\%$ ID noise compared with MLC.}

\begin{table}[]
\centering
 \caption{\hl{Testing Acc.(\%) on CIFAR-10 and CIFAR-100 with varying ratios of instance-dependent noise.}} %\textbf{Resnet18}}
 \label{tab:inst}
\begin{tabular}{|lcccc|}
\hline
\textbf{Dataset }     & \multicolumn{2}{c}{\textbf{CIFAR-10}}                          & \multicolumn{2}{c|}{\textbf{CIFAR-100}}                         \\
\textbf{Noise ratio } & \textbf{0.2}              & \textbf{0.4}              & \textbf{0.2}              & \textbf{0.4}              \\\hline\hline
\textbf{PTD}~\citep{xia2020part} & 76.05 & 58.62 &-&-\\
\textbf{Decoupling}~\citep{malach2017decoupling}   & 77.85                     & 59.05                     & 48.33                     & 34.26\\
\textbf{MentorNet}~\citep{jiang2018Mentornet}    & 79.12                     & 70.27                     & 51.73                     & 40.90  \\
\textbf{Co-teaching}~\citep{han2018co}  & 86.54                     & 80.98                     & 57.24                     & 45.69   \\
\textbf{DMI}~\citep{xu2019l_dmi}          & 89.14                     & 84.78                     & 58.05                     & 47.36  \\
\textbf{T-revision}~\citep{xia2019anchor}   & 89.46                     & 85.37                     & 60.71     & 51.54 \\\hline\hline
\textbf{GLC}~\citep{hendrycks2018using}          & 87.81                     & 82.19                     & 59.79        & 50.96     \\
\textbf{MWNet }~\citep{shu2019meta}       & 88.91      & 84.77                     & 63.74                     & 55.27                     \\
\textbf{MLC}~\citep{wang2020training}          & 89.16       & 85.11                     & 63.14         & 56.76        \\\hline
\textbf{WarPI (Detc.)} & 89.27                     & 87.01                     & 64.92                     & 56.94                     \\
\textbf{WarPI}        & \textbf{89.76}            &\textbf{ 87.57}            & \textbf{65.08  }          & \textbf{57.38}            \\\hline
\end{tabular}
\end{table}


\begin{table}[]\small
  \centering
  \caption{Testing Acc.(\%) on Clothing1M.}
     \label{tab:cloth}
  \begin{tabular}{|lcc|}
\hline
\textbf{Method}    &\textbf{Year}   & \textbf{Test Acc.} \\ \hline\hline
% \textbf{Joint Learning}~\citep{tanaka2018joint}                   &72.23\\
\textbf{Base Model} &- & 68.94\\
\textbf{Co-teaching}$^*$~\citep{han2018co} &2018 &  69.21 \\
\textbf{Co-teaching+}$^*$~\citep{yu2019does}  &2019 &  59.32  \\
\textbf{LCCN}~\citep{yao2019safeguarded}     &2019              & 73.07    \\
\textbf{MLNT}~\citep{li2019learning}       &2019             & 73.47    \\
\textbf{PENCIL}~\citep{yi2019probabilistic}      &2019            & 73.49   \\
% \textbf{GLC}~\citep{hendrycks2018using}                    &73.69\\
\textbf{MWNet}~\citep{shu2019meta}        &2019          & 73.72    \\
\textbf{JoCoR}~\citep{wei2020combating} &2020 & 70.30\\ 
\textbf{DivideMix}~\citep{li2020dividemix}      &2020         & 74.76    \\
\textbf{LIMITL}~\cite{harutyunyan2020improving} &2020 & 71.39\\
\textbf{ELR+}~\citep{liu2020early}        &2020            & 74.81 \\    
\textbf{PTD-R-V}~\citep{xia2020part}  &2020     & 71.67   \\ 
\textbf{CAL}~\citep{Zhu_2021_CVPR} &2021 & 74.17\\ 
\textbf{PLC}~\citep{zhang2021learning}  &2021     & 73.24    \\ \hline
\textbf{WarPI (Detc.)}& -& 74.41    \\
\textbf{WarPI}                & - & \textbf{74.98}   \\
\hline
\end{tabular}
\begin{tablenotes}
        \footnotesize
        \item[1] \qquad\qquad\qquad\qquad\qquad \quad * results from \citep{wei2020combating}.
\end{tablenotes}
\end{table}%


\textbf{Open-set Noise}. To verify the effectiveness of the model for handling open-set noise, we evaluate it on challenging real-world datasets, \textit{i.e.}, Clothing1M and Food-101N. In contrast to pre-defining a clean meta dataset in CIFAR-10 and CIFAR-100, these two real-world datasets contain the clean validation set. For the fair comparison, we utilize the same architecture~\citep{shu2019meta,zhang2021learning} of ResNet-50 pre-trained on ImageNet. We compare our proposed method with most of the recent representative approaches as shown in Table \ref{tab:cloth} and \ref{tab:food}. Our WarPI achieves new state-of-the-arts of 74.98 on Clothing1M and 85.91 on Food-101N. Moreover, compared with the meta-learning methods (\textit{e.g.}, MWNet), we achieve significant improvement of $1.26\%$ on Clothing1M and $1.19\%$ on Food-101N.  

%test the advanced nature of our method through multiple sets of experiments. The experiment that follows focuses on three areas: 
%(1) We demonstrated the superiority of our approach over previous superior performance approaches by comparing accuracy in a variety of noise environments. (2) We proved the positive impact of adding probabilistic model to the model through ablation experiments. (3) We explored the effect of the number of Monte Carlo sampling in WarPI on results. All method in this paper are repeated 3 times with different random seeds and results are averaged.


%Table.1 shows the performance of our method in FLIP. It’s clear that our method obtain the best performance with multiple noise ratios in both datasets. Under $0\%$ noise ratio, the accuracy of our method slightly worse than Focal loss~\citep{lin2017focal} and Fine-tining. At a noise ratio of $20\%$ for CIFAR100, the performance is second only to MLSG~\citep{algan2021meta}.  Meanwhile, we compare the impact of adding probabilistic inference to WarPI on model performance. It can be seen that the way of sampling make a positive contribution to the model. As the proportion of sample noise increases from $0\%$ to $40\%$, the accuracy of our method increases even more significantly compared to the previous methods, which demonstrates the robustness of our approach under noise labels.



\begin{table}[]\small
\centering
\caption{Testing Acc.(\%) on Food-101N.}
   \label{tab:food}
\begin{tabular}{|lcc|}
\hline
\textbf{Method}  &\textbf{Year}  & \textbf{Test Acc.} \\ \hline\hline
\textbf{Base Model} &- & 81.67    \\
\textbf{CleanNet} (hard)~\citep{lee2018cleannet}  &2018 & 83.47    \\
\textbf{CleanNet} (soft)~\citep{lee2018cleannet}  &2018 & 83.95    \\
\textbf{MWNet}~\citep{shu2019meta}  &2019   & 84.72 \\
\textbf{SMP}~\citep{han2019deep} &2019 & 85.11\\
\textbf{NoiseRank}~\citep{sharma2020noiserank} &2020& 85.20\\
\textbf{PLC}~\citep{zhang2021learning}  &2021     & 85.28    \\ \hline 
\textbf{WarPI (Detc.)} &-& 85.40    \\
\textbf{WarPI}    &- &\textbf{85.91} \\
\hline
\end{tabular}
\end{table}




\subsection{Further Analysis}
We provide further analysis for the proposed WarPI in three aspects of effectiveness, efficiency, and stability.




\textbf{Effectiveness}. We plot the distribution of cross-entropy losses for training samples in Figure \ref{fig:dist} after finishing training the model. The bar shows the number of the sample whose loss fall into a certain interval. The blue bar represents the loss computed directly from the output of the classification network, while the red one is the loss computed from the logits rectified by the warped vector generated with our meta-network. As shown in Figure \ref{fig:dist}, the rectified loss is obviously lower than the original one in all intervals. \hl{Meanwhile, the number of samples with a relatively higher loss value increases as the noise ratio rises. According to the observation}~\citep{zhang2018generalized} \hl{that the low-confident sample with higher loss is more likely corrupted, our meta-network can alleviate the negative impact of the classification network from noisy labels. Therefore, minimizing the rectified loss can achieve good generalization performance for noisy labels.} To achieve a better visualization for the virtue of our meta-network, we draw the initialized and estimated confusion matrices for constructing asymmetric noisy data on CIFAR-10 in Figure \ref{fig:confusion_matrix}. By using the rectified prediction for each training sample, our model almost achieves the unbiased estimation for the initialized confusion matrix. 



\begin{figure}[]
\centering
\includegraphics[width=12cm]{figs/num_of_loss.pdf}
\caption{The loss distribution on training data under 20$\%$ and 40$\%$ asymmetric noise on CIFAR-10. WarPI can alleviate the negative impact of corrupted labels.}
\label{fig:dist}
\end{figure}


\begin{figure}[]
\centering
\begin{minipage}[b]{0.99\linewidth}
\includegraphics[width=13cm]{figs/matrix_cifar10_flip0.2.pdf}
\end{minipage}
\quad
\begin{minipage}[b]{0.99\linewidth}
\includegraphics[width=13cm]{figs/matrix_cifar10_flip0.4.pdf}
%\caption{Sad Smiley}
%\label{fig:minipage2}
\end{minipage}
\caption{\hl{The estimated confusion matrices for asymmetric noise with $20\%$ (Top) and $40\%$ (Bottom). Our model almost achieves the unbiased estimation for the initialized confusion matrix.}}
\label{fig:confusion_matrix}
\end{figure}


\textbf{Efficiency}. The sampling number for the rectifying vector has important impact on performance and efficiency. We conduct experiments on CIFAR-10 and CIFAR-100 with variant sample numbers for rectifying vectors. As demonstrated in Figure \ref{fig:ell}, the testing accuracy turns to be higher, then keeps stable as the number of samples increasing. Despite the fact that the generalization ability improves given more samples, the training time for each epoch increases linearly. To balance performance and efficiency, we set $\ell$ as $10$ for toy datasets of CIFAR-10 and CIFAR-100. \hl{As for large-scale real-world datasets, the predictive posterior can be also estimated accurately with $\ell=1$ given sufficient samples, which is illustrated in Table} \ref{fig:ell} \hl{ where the batch size keeps 32 for all experiments.} Therefore, our model reaches high accuracy and meanwhile keeps efficient on Clothing1M and Food-101N. 
%with $0.4$ noise ratio.
%We explore the impact of the number K of sampling taken from latent variable on the predictive effect of the model. The final results we show in Figure.3. It is clear that a higher number of sampling gives a better performance of the probabilistic inference in WarPI.







%Figure.4 shows the label distribution matrix under $40\%$ of the wrong labels under CIFAR10. The logits vector obtained by classification network for all images are processed by WarPI and then a new label predicition matrix is obtained. After WarPI, we attach a transfer vector to the prediction vector of classification network output, so that the loss generated by noise label becomes smaller and its impact on classification network is minimized. The new matrix that closely approximates the initial confusion matrix proves the validity of WarPI.\\



\begin{figure}[]  
\centering  
\includegraphics[width=12cm]{figs/plot_of_TimeANDacc.pdf} 
\caption{Generalization performance and convergence speed as the sample number increases. We consider $\ell=10$ to achieve a good trade-off between performance and training time.}
\label{fig:ell}  
\end{figure} 


\begin{table}[]
	\centering
	\caption{\hl{Testing Acc.(\%) and computation cost (seconds per batch) on Clothing1M and Food-101N.}}
	\label{tab:ell}
	\begin{tabular}{l|cc|cc}
		\hline\hline
		% \textbf{Noise Type} & \multicolumn{4}{c}{Flip}                                                                                \\ \hline
		\textbf{Dataset}                         & \multicolumn{2}{c|}{Clothing1M}                         & \multicolumn{2}{c}{Food-101N}                   \\ \hline
		\textbf{Results}                     & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c|}{sec./batch} & \multicolumn{1}{c}{Acc.} & sec./batch       \\ \hline\hline
		$\ell$=1                        & 74.98              & 1.9                &85.91                & 1.7   \\
		$\ell$=4      & 75.04                 & 4.6                & 85.95                & 4.2  \\ \hline\hline
	\end{tabular}
\end{table}



%To verify the actual impact of our method on label noise dataset, we fed weak data(CIFAR10 with 40$\%$ noise label) into a robust model that could make correct classification. The result is in line with our expectation that the noise data has a large loss and the correctly labelled sample has a small loss. We use WarPI to learn a vector attached to logits after this classification network. Its effect is as obvious as the one shown in Figure.6. The loss generated by the wrong sample is effectively reduced. During training, It's clear that WarPI reduces the impact of mislabelling on classification model.






\textbf{Stability}. WarPI armed with probabilistic inference demonstrates superior generalization ability as the number of epoch increases. As illustrated in Figure \ref{fig:stable}, the testing accuracy for MWNet and the deterministic model decreases heavily as the training proceeds. Furthermore, their increment trends of loss on meta-data indicate the classification network turns to overfit to noisy labels. This is in contrast to WarPI where it still keeps high testing accuracy even after 200 epochs. WarPI exhibits great propriety of overcoming overfitting to noisy data and achieves favorable generalization performance on robust learning. 






\begin{figure}[]
\centering
\begin{minipage}[b]{0.48\linewidth}
\includegraphics[width=6.5cm]{figs/test_acc.pdf}
%\caption{Happy Smiley}
%\label{fig:minipage1}
\end{minipage}
\quad
\begin{minipage}[b]{0.48\linewidth}
\includegraphics[width=6.5cm]{figs/meta_loss.pdf}
%\caption{Sad Smiley}
%\label{fig:minipage2}
\end{minipage}
\caption{The test accuracy and meta loss of the deterministic model, WarPI, and MWNet under the case of $40\%$ noise ratio on CIFAR-10. Compared to the deterministic model and MWNet, WarPI can avoid overfitting demonstrating favorable generalization ability. (Best viewed in color)}
\label{fig:stable}
\end{figure}























==> 6-conclusion.tex <==

In this paper, we propose to learn to adaptively rectify the training process under the meta-learning scenario. By formulating the learning process as a hierarchical probabilistic model and considering the rectifying vector as a latent variable, we propose warped probabilistic inference (WarPI) to achieve effective estimation for the predictive posterior. Our framework consists of the meta-network and classification network. For the meta-network, we adopt the idea of amortization that directly generates the posterior distribution by a shared neural network, achieving fast inference during forward propagation. Unlike the existing method to directly approximate the weighting function, our meta-network is learned to estimate a rectifying vector from the input of the logits and labels, which has the capability of leveraging sufficient information lying in them. We conduct extensive experiments on four datasets, \textit{i.e.}, CIFAR-10, CIFAR-100, Clothing1M, and Food-101N under three types of noise. The proposed WarPI achieves state-of-the-art on all benchmarks and consistently outperforms those deterministic models using meta-data. Exhaustive analysis of effectiveness, efficiency, and stability exhibits the virtue of our model for robust learning tasks.  




\section*{Acknowledgements}
This research was supported in part by Natural Science Foundation of China (No. 61876098, 6210021184) and China
Postdoctoral Science Foundation (No. 2021TQ0195).

==> 8-resume.tex <==

\noindent\textbf{Haoliang Sun} received PhD and B.E from Shandong University in 2014 and 2020, respectively. He had been a visiting student at University of Western Ontario, CA and University of Wisconsin-Madison, USA. He currently pursues the postdoc at Shandong University. His research interests include machine learning, computer vision, and medical image analysis.
\\

\noindent\textbf{Chenhui Guo} received B.E from Shandong University in 2020. She is now pursuing the master's degree at Shandong University. Her research interests include machine learning and data mining.
\\

\noindent\textbf{Qi Wei} received B.E from Wuhan University of Science and Technology in 2020. He is now pursuing the master's degree at Shandong University. His research interests include machine learning and data mining.
\\

\noindent\textbf{Zhongyi Han} received his B.Eng. and M.M. degree from Shandong University of Traditional Chinese Medicine, in 2016 and 2019, respectively. He had been a visiting student at University of Western Ontario, CA. Currently, he is working toward a Ph.D. degree with the Artificial Intelligence Research Center in Shandong University, supervised by Prof. Yilong Yin. His research interest is mainly in machine learning and data mining. He has published over 10 papers in leading international journals and conferences.
\\

\noindent\textbf{Yilong Yin} received the Ph.D. degree from Jilin University, Changchun, China, in 2000. From 2000 to 2002, he was a Postdoctoral Fellow with the Department of Electronic Science and Engineering, Nanjing University, Nanjing, China. He is the Director of the Artificial Intelligence Research Center and the Professor of Shandong University, Jinan, China. His research interests
include machine learning and data mining. He
has published over 100 papers in leading international
journals and conferences.
